Beyond Backprop: Online Alternating Minimization with Auxiliary Variables

Despite significant recent advances in deep neural networks, training them remains a challenge due to the highly non-convex nature of the objective function. State-of-the-art methods rely on error backpropagation, which suffers from several well-known issues, such as vanishing and exploding gradients, inability to handle non-differentiable nonlinearities and to parallelize weight-updates across layers, and biological implausibility. These limitations continue to motivate exploration of alternative training algorithms, including several recently proposed auxiliary-variable methods which break the complex nested objective function into local subproblems. However, those techniques are mainly offline (batch), which limits their applicability to extremely large datasets, as well as to online, continual or reinforcement learning. The main contribution of our work is a novel online (stochastic/mini-batch) alternating minimization (AM) approach for training deep neural networks, together with the first theoretical convergence guarantees for AM in stochastic settings and promising empirical results on a variety of architectures and datasets.

==> extra_dict.tex <==
--------------- extra stuff ---------
 
However, offline (batch) learning performing optimization with respect to the potentially very large training dataset is not scalable.  Moreover, we would like to have an online approach which can adapt to a continuous stream of data in a lifelong learning setting. We build our approach on top of the  {\em online dictionary learning (ODL)} proposed in \cite{mairal2009online}. In \cite{mairal2009online}, we assume that, at $t$-th iteration of the algorithm, we obtain a sample $\bx_t$ (or a mini-batch of samples), which is first encoded into   ${\bf c}_t$ using the dictionary ${\bf D}_{t-1}$ from the previous iteration; then the dictionary update step is optimizing a following   {\em surrogate} objective function $\hat{f}_n(D)=$
\begin{eqnarray}
%\label{eqn:dic_learn_objective}
   \frac{1}{n} \sum_{t=1}^N \frac{1}{2} || \bs{x}_t - \bs{D} \bs{c}_t ||_2^2 + \lambda_{c} || \bs{c}_t ||_1,
\vspace{-0.05in}
\end{eqnarray}
where each 
\begin{eqnarray}
\bs{c}_t = \arg \min_{\bs{c}} \frac{1}{2} || \bs{x}_t - \bs{D_{t-1}} \bs{c} ||_2^2 + \lambda_{c} || \bs{c} ||_1.
\label{eq:Lasso}
\end{eqnarray}
The surrogate objective is similar to the
 original one  in eq. \eqnref{eqn:dic_learn_objective}, for  $n=N$, except for an important change: in eq. \eqnref{eqn:dic_learn_objective}, each code $\bs{c}_t$ is computed using the {\em same} dictionary $\boldsymbol{D}$, while  the surrogate function keeps the codes
  $\bs{c}_t$ %, \bs{\alpha}_2, \cdots, \bs{\alpha}_{t}$
   from the {\em previous} iterations, computed using the corresponding previous dictionaries,
 i.e.  {\em does not recompute} the  codes of  previously
  seen samples after each dictionary update.
  This speeds up the learning without worsening the (asymptotic) performance, since
 the surrogate objective   converges to the original one in \eqnref{eqn:dic_learn_objective}, under certain assumptions, including data stationarity  \cite{mairal2009online}.
 
 
 


We assuming the   loss functions $l^p$ and $l^r$ which correspond to the type of variables being reconstructed or predicted (i.e., real-valued variables are assumed to be Gaussian and associated with the sum-squared loss as in classical sparse coding, and the class label is typically a categoric variable associated with multinomial, or cross-entropy,  loss), e.g. 
    $ l^r ( {\bf D^{ij}},{\bf c^i}|{\bf c^j}) = ||{\bf c^j} -  D^{ij}{\bf c^i}||^2_2,$ and 
 $l^p ({\bf W^{i k+1}}, {\bf y}|{\bf c^i})    = multinomial ~ loss$.
 
  The algorithm for {\em online supervised deep dictionary learning} is shown in \algoref{alg:ODSDL}, assuming the architecture in Figure 1 (to be included: a multilayer model combining k levels of deep dictionary with the top supervised layer).
  
%\input{sec_alg_bullet_points.tex}
\input{sec_AltMin_algorithm.tex}
  
At each iteration $t$, the next input sample $\bs{x}_t$  (or a batch of samples) is obtained. For each layer of hidden variables, $i$, from 1 to k,  we first obtain a sparse code ${\bf c}^i_t$  
 by solving via proximal method the objective in step \ref{as:sparse_coding}, assuming fixed dictionaries $\bs D^{i,0}$ and  $\bs D^{i,i-1}$ and fixed predictive weights $\bs W^{i,k+1}$.
Next,   both dictionaries are updated.

\noindent{\bf Dictionary update.} Let $\bs D$ denote $\bs D^{i,0}$ and  $\bs D^{i,i-1}$ at their update steps, respectively.  Note that, in order to prevent the dictionary entries from growing arbitrarily large, we follow \cite{mairal2009online} and impose the norm constraint, i.e. keep
  the columns of $\bs{D}$ within the convex set  $\mathcal{C}= \{\boldsymbol{D} \in \mathbb{R}^{m \times k} $ $~~s.t.~~ \forall j~ \boldsymbol{d}^T_j \boldsymbol{u}_j \leq 1 \}$. To update each dictionary, we optimize  the following {\em surrogate} objective function $\hat{f}_t({\bf D})$\footnote{this function is called surrogate since  each of the codes obtained on previous iterations $j < t$ are obtained using the corresponding earlier versions of the dictionary, rather than being computed with respect to the most recent dictionary, as in offline setting, and thus the surrogate function in online setting approximates the corresponding version in offline setting.}: 
%\vspace{-0.01in}
\begin{small}
\begin{equation}
\label{eqn:optimize_dict_obj_group_sparse}
\min_{\boldsymbol{D} \in \mathcal{C}}
\frac{1}{t} \sum_{j=1}^t \frac{1}{2}
||
\bs{c}^{i-1}_j - \boldsymbol{D} {\bs c}^i_j
||_2^2
+
\lambda_g \sum_j ||\boldsymbol{d}_j||_2
+
\sum_j\lambda_j||\boldsymbol{d}_j||_1.
%\vspace{-0.01in}
\end{equation}
\end{small}
Again, following \cite{mairal2009online}, we rewrite the above objective using the fact that $\min_{\boldsymbol{D} \in \mathcal{C}} \frac{1}{t}
\sum_{i=1}^t \frac{1}{2} ||
\boldsymbol{x}_i - \boldsymbol{D} \boldsymbol{\alpha}_i
||_2^2  $ is equivalent to   
\vspace{-0.05in}
\begin{eqnarray}
\label{eqn:optimize_dict_obj}
  \min_{\boldsymbol{D} \in \mathcal{C}}
\frac{1}{t} \big ( \frac{1}{2}
Tr(\boldsymbol{D}^T\boldsymbol{D}\boldsymbol{A}) - Tr(\boldsymbol{D}^T\boldsymbol{B}) \big ),
%\vspace{-0.02in}
\vspace{-0.05in}
\end{eqnarray}
  where $\bs{A} = \sum_{i=1}^t \boldsymbol{\alpha}_i \boldsymbol{\alpha}_i^T$ and $\bs{B} = \sum_{i=1}^t \boldsymbol{x}_i \boldsymbol{\alpha}_i^T$ are the ``bookkeeping''
  matrices (we also call them ``memories'' of the model), compactly representing the input samples and encoding history.
   At each iteration, once the new input sample $\boldsymbol{x}_i $ is encoded,
    the matrices are updated as $\boldsymbol{A} \gets \boldsymbol{A} + \boldsymbol{\alpha}_t \boldsymbol{\alpha}_t^T$ and $\boldsymbol{B}
\gets
\boldsymbol{B} + \boldsymbol{x}_t \boldsymbol{\alpha}_t^T$ (see the step \ref{as:memory_update}  of \algoref{alg:ODSDL}).
We follow \cite{mairal2009online} and use a \emph{block coordinate descent}   to optimize
 the convex objective
 in eq. \ref{eqn:optimize_dict_obj}; it iterates over the dictionary elements in a fixed sequence, until convergence, optimizing each while
 keeping the others fixed as shown in eq. \eqnref{eqn:dict_update}  and \ref{as:dict_element_normalize}  in \algoref{alg:ODSDL},
 except that, in our approach,
$\boldsymbol{u}_j$ is transformed into $\boldsymbol{w}_j$   to impose an additional regularizer before computing step \ref{as:dict_element_normalize}).
 
\begin{align}
\label{eqn:dict_update}
&
%\underbrace{
\boldsymbol{u}_j
\gets
\frac{
	\boldsymbol{b}_j
	-
	 \sum_{k \not = j} \boldsymbol{d}_k  a_{jk}
}
{
	a_{jj}
}
%}_{\text{minimize the least square error}}
;\ \ \
%\underbrace{
\boldsymbol{d}_j
\gets
\frac{
	\boldsymbol{u}_j
}
{
	\max(1, ||\boldsymbol{u}_j||_2)
}
\end{align}
 
\noindent{\bf Updating predictive weights $W^{i,k+1}$.} Finally,  step \ref{as:updateW}  in \algoref{alg:ODSDL} updates predictive (forward) weights ${\bf W}^{i,k+1}$ by fitting multinomial regression from code ${\bf c}^i_t$ to ${\bf y}_t$. Note that we have no obvious way to express the multinomial loss in terms of memory matrices as it was done for the sum-squared loss in eq. \ref{eqn:optimize_dict_obj}, and thus we will be using SGD instead of block-coordinate descent for this part of the loss function.

==> math_commands.tex <==
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\newsetminus}{{\!-\!}}
\newcommand{\cVmA}{{\cV\newsetminus\cA}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cs}{s}
\newcommand{\cVms}{{\cV-\cs}}

\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\resid}{\cR}

\newcommand{\NP}{{\mathbf{NP}}}

% \DeclareMathOperator{\MIF}{MI} 

\newcommand{\bs}[1]{\boldsymbol{#1}}


\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{(\ref{#1})}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\prcref}[1]{Procedure~\ref{#1}}
\newcommand{\assmref}[1]{Assumption~\ref{#1}}
\newcommand{\crlref}[1]{Corollary~\ref{#1}}
\newcommand{\algoref}[1]{Alg.~\ref{#1}}
\newcommand{\prpref}[1]{Proposition~\ref{#1}}
\newcommand{\cnjref}[1]{Conjecture~\ref{#1}}
\newcommand{\axmref}[1]{Axiom~\ref{#1}}
\newcommand{\lmaref}[1]{Lemma~\ref{#1}}

%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}[lemma]{Theorem}
%\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{procedure}[lemma]{Procedure}
\newtheorem{assumption}[lemma]{Assumption}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{conclusion}[lemma]{Conclusion}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{conjecture}[lemma]{Conjecture}
\newtheorem{axiom}[lemma]{Axiom}
\newtheorem{algo}[lemma]{Algorithm}

\newcommand{\mai}{ODL }
\newcommand{\nmai}{NODL+ }
\newcommand{\gmai}{NODL- }
\newcommand{\ngmai}{NODL }
%
\newcommand{\mains}{ODL}
\newcommand{\nmains}{NODL+}
\newcommand{\gmains}{NODL-}
\newcommand{\ngmains}{NODL}

%additions suggested by Sahil
\newcommand{\s}[1]{\textcolor{magenta}{#1}}
%deletions suggested by Sahil
\newcommand{\sd}[1]{\textcolor{orange}{#1}}


==> sec_ODSDL_2pass_algorithm.tex <==
%\vspace{-0.05in}
\begin{small}
\begin{algorithm}[tbh]
\caption{
%\fontsize{9}{9}\selectfont
 Online Deep Supervised Dictionary Learning (ODSDL)
}
\csize
\begin{algorithmic}[1]
\STATE
{\bf Input}: Data stream $\boldsymbol{x}_1, \bs{x}_2, \cdots, \bs{x}_n \in \mathbb{R}^{m_0}$, and corresponding class label {\em vectors} $\boldsymbol{y}_1, \bs{y}_2, \cdots, \bs{y}_n \in \mathbb{R}^{m_{k+1}}$;  $m_i$ is the number of nodes at $i$-th level; sparsity parameter for  dictionary elements, $\lambda_d$; sparsity parameter for  code, $\lambda_c$;
group sparsity regularization parameter, $\lambda_g$;
initial  {\em reconstructive weights  } $\boldsymbol{D^{i, i-1}} \in \mathbb{R}^{m_{i-1} \times m_{i}}$ in dictionaries for reconstructing  layer $i-1$ from layer $i$, for $i = 1,...,L$;
initial {\em predictive weights}  $\boldsymbol{W^{i, L+1}} \in \mathbb{R}^{m_{i} \times m_{L+1}}$,  for predicting the labels (layer $L+1$) from the layer $i$ variables, for $i = 1,...,L$.
%\newline
\STATE
{\bf Initialize}:  \COMMENT{ reset the ``memory matrices''}
\FOR{ $i = 1$ to $k$}
\STATE $\bs{A}^{i,0} \gets 0$,
$\bs{A}^{i,i-1} \gets 0$, $\bs{B}^{i,0} \gets 0$, $\bs{B}^{i,i-1} \gets 0$~   
\ENDFOR
%\WHILE{there is a batch of data to process}
\FOR{$t = 1$ to $n$}
%\STATE
%{\bf Input} next batch  of data $\{ \boldsymbol{x}_1, \cdots,  \boldsymbol{x}_t, \cdots, \boldsymbol{x}_b \}$  \\
\STATE
Input $\boldsymbol{x}_t$ %\COMMENT{ the $t_{th}$ batch of data}
\label{as:input_data}
\FOR{$i=1$ to $L$}
\STATE \COMMENT{Supervised sparse coding: forward pass}\\
$
 {\bs c}^i_t = \arg \min_{\bs c \in \mathbb{R}^{m_i}} \sum_{j \in \{0,i-1\}}
  ||{\bf c}^j - {\bf D}^{i,j}{\bf c}^i|||^2_2 ~ + ~~$  
 % $||{\bf c}^i -  {\bf D}^{i+1, i}{\bf c}^{i+1 }||^2_2 +  
 $ \alpha    
  l^p ({\bf W}^{i, L+1}, {\bf y}|{\bf c}^i) +  \lambda_{c}  ||\bs {c}||_1.  
$
\label{as:sparse_coding1}
\ENDFOR
\FOR{$i=L$ to $1$}
\STATE \COMMENT{Supervised sparse coding: backward pass }\\
$
 {\bs c}^i_t = \arg \min_{\bs c \in \mathbb{R}^{m_i}} \sum_{j \in \{0,i-1\}}
  ||{\bf c}^j - {\bf D}^{i,j}{\bf c}^i|||^2_2 ~ + ~~$  
 $ ||{\bf c}^i -  {\bf D}^{i+1, i}{\bf c}^{i+1 }||^2_2 +  
  \alpha    
  l^p ({\bf W}^{i, L+1}, {\bf y}|{\bf c}^i) +  \lambda_{c}  ||\bs {c}||_1.  
$
\label{as:sparse_coding2}
\ENDFOR
\FOR{$i=1$ to $L$}
\STATE \COMMENT{Memory matrices updates: }\\
$
\bs{A}^{i,0} \gets \bs{A}^{i,0} + \bs{c}^i_t {\bs{c}^i_t}^T,~
$
$
\bs{B}^{i,0} \gets \bs{B}^{i,0} + \bs{x}_t {\bs{c}^i_t}^T,~
$ \\
$
\bs{A}^{i,i-1} \gets \bs{A}^{i,i-1} + \bs{c}^i_t {\bs{c}^i_t}^T
$,~
$
\bs{B}^{i,i-1} \gets \bs{B}^{i,i-1} + \bs{c}^{i-1}_t {\bs{c}^i_t}^T
$ 
\label{as:memory_update}
\FOR{$j=0$ and $j={i-1}$} 
\STATE
{\bf updateDictionary}($\bs{D}^{i,j},\bs{A}^{i,j},\bs{B}^{i,j}$)
\label{as:updateD}
\ENDFOR
\STATE {\bf fitMultiNomial}($\bs{W}^{i,k+1},{\bs c}^i, {\bs y}$)
\label{as:updateW}
\ENDFOR
\ENDFOR
\RETURN $\bs{D},\bs{W}$ 
\end{algorithmic}

\begin{algorithmic}[1]
\STATE \COMMENT{--------------------------------------------}
\STATE {\bf function updateDictionary}($\bs{D}^{i,j},\bs{A}^{i,j},\bs{B}^{i,j}$)
\REPEAT
%\COMMENT{Update each dictionary element:}
\FOR{$j = 1$ to $k$}
\STATE
$
\boldsymbol{u}_j
\gets
\frac{
	\boldsymbol{b}_j
	-
	 \sum_{k \not = j} \boldsymbol{d}_k  a_{jk}
}
{
	a_{jj}
}
$
\label{as:dict_element_compute}
%\\
%&
%\algshade{
\\
\algshade{
\STATE
%\begin{align*}
%\begin{align*}
$
\boldsymbol{v}_j
\gets
Prox_{\lambda_j ||.||_1}(\boldsymbol{u}_j)
=
sgn(\boldsymbol{u}_j) (|\boldsymbol{u}_j| - \lambda_j)_{+},
$
%\COMMENT{$\lambda_j$ tuned to get $\beta_d$ non-zeros in $\boldsymbol{v}_j$}
\COMMENT{Sparsity}
\label{as:sparse_elements}
%}
%\\
%&
\\
%\algshade{
\STATE
$
\boldsymbol{w}_j
\gets
\boldsymbol{v}_j
\left(
	1
	-
	\frac{\lambda_g}{||\boldsymbol{v}_j||_2}
\right)_{+} 
$
\COMMENT{ $l_1/l_2$ group sparsity}
}
\label{as:kill_elements}
\\
\STATE
$
\boldsymbol{d}_j
\gets
\frac{
	\boldsymbol{w}_j
}
{
	\max(1, ||\boldsymbol{w}_j||_2)
}	
$
\label{as:dict_element_normalize}
\ENDFOR
\UNTIL{\textbf{convergence}}
\RETURN $\bs{D}^{i,j},\bs{A}^{i,j},\bs{B}^{i,j}$
%\label{as:dict_update_until_converge}
\end{algorithmic}
\label{alg:ODSDL}
\end{algorithm}
\end{small}
%\vspace{-0.05in}


==> sec_ONN_AltMIN.tex <==
%\vspace{-0.05in}
\begin{small}
\begin{algorithm}[tbh]
\caption{
%\fontsize{9}{9}\selectfont
 Online Deep Supervised Dictionary Learning (ODSDL)
}
\csize
\begin{algorithmic}[1]
\STATE
{\bf Input}: Data stream $\boldsymbol{x}_1, \bs{x}_2, \cdots, \bs{x}_n \in \mathbb{R}^{m_0}$, and corresponding class label {\em vectors} $\boldsymbol{y}_1, \bs{y}_2, \cdots, \bs{y}_n \in \mathbb{R}^{m_{k+1}}$;  $m_i$ is the number of nodes at $i$-th level; sparsity parameter for  dictionary elements, $\lambda_d$; sparsity parameter for  code, $\lambda_c$;
group sparsity regularization parameter, $\lambda_g$;
initial  {\em reconstructive weights  } $\boldsymbol{D^{i, i-1}} \in \mathbb{R}^{m_{i-1} \times m_{i}}$ in dictionaries for reconstructing  layer $i-1$ from layer $i$, for $i = 1,...,L$;
initial {\em predictive weights}  $\boldsymbol{W^{i, L+1}} \in \mathbb{R}^{m_{i} \times m_{L+1}}$,  for predicting the labels (layer $L+1$) from the layer $i$ variables, for $i = 1,...,L$.
%\newline
\STATE
{\bf Initialize}:  \COMMENT{ reset the ``memory matrices''}
\FOR{ $i = 1$ to $k$}
\STATE $\bs{A}^{i,0} \gets 0$,
$\bs{A}^{i,i-1} \gets 0$, $\bs{B}^{i,0} \gets 0$, $\bs{B}^{i,i-1} \gets 0$~   
\ENDFOR
%\WHILE{there is a batch of data to process}
\FOR{$t = 1$ to $n$}
%\STATE
%{\bf Input} next batch  of data $\{ \boldsymbol{x}_1, \cdots,  \boldsymbol{x}_t, \cdots, \boldsymbol{x}_b \}$  \\
\STATE
Input $\boldsymbol{x}_t$ %\COMMENT{ the $t_{th}$ batch of data}
\label{as:input_data}
\FOR{$i=1$ to $L$}
\STATE \COMMENT{Supervised sparse coding: forward pass  (ignoring the forward links from undefined $c^{i+1}$ to $c^i$) }\\
$
 {\bs c}^i_t = \arg \min_{\bs c \in \mathbb{R}^{m_i}} \sum_{j \in \{0,i-1\}}
  ||{\bf c}^j - {\bf D}^{i,j}{\bf c}^i|||^2_2 ~ + ~~$  
  $||{\bf c}^i -  {\bf D}^{i+1, i}{\bf c}^{i+1 }||^2_2 +  
  \alpha    
  l^p ({\bf W}^{i, L+1}, {\bf y}|{\bf c}^i) +  \lambda_{c}  ||\bs {c}||_1.  
$
\label{as:sparse_coding1}
\ENDFOR
\FOR{$i=L$ to $1$}
\STATE \COMMENT{Supervised sparse coding: backward pass  (now including the forward links from  $c^{i+1}$ to $c^i$) }\\
$
 {\bs c}^i_t = \arg \min_{\bs c \in \mathbb{R}^{m_i}} \sum_{j \in \{0,i-1\}}
  ||{\bf c}^j - {\bf D}^{i,j}{\bf c}^i|||^2_2 ~ + ~~$  
  %$||{\bf c}^i -  {\bf D}^{i+1, i}{\bf c}^{i+1 }||^2_2 +  
 $ \alpha    
  l^p ({\bf W}^{i, L+1}, {\bf y}|{\bf c}^i) +  \lambda_{c}  ||\bs {c}||_1.  
$
\label{as:sparse_coding2}
\ENDFOR
\FOR{$i=1$ to $L$}
\STATE \COMMENT{Memory matrices updates: }\\
$
\bs{A}^{i,0} \gets \bs{A}^{i,0} + \bs{c}^i_t {\bs{c}^i_t}^T,~
$
$
\bs{B}^{i,0} \gets \bs{B}^{i,0} + \bs{x}_t {\bs{c}^i_t}^T,~
$ \\
$
\bs{A}^{i,i-1} \gets \bs{A}^{i,i-1} + \bs{c}^i_t {\bs{c}^i_t}^T
$,~
$
\bs{B}^{i,i-1} \gets \bs{B}^{i,i-1} + \bs{c}^{i-1}_t {\bs{c}^i_t}^T
$ 
\label{as:memory_update}
\FOR{$j=0$ and $j={i-1}$} 
\STATE
{\bf updateDictionary}($\bs{D}^{i,j},\bs{A}^{i,j},\bs{B}^{i,j}$)
\label{as:updateD}
\ENDFOR
\STATE {\bf fitMultiNomial}($\bs{W}^{i,k+1},{\bs c}^i, {\bs y}$)
\label{as:updateW}
\ENDFOR
\ENDFOR
\RETURN $\bs{D},\bs{W}$ 
\end{algorithmic}

\begin{algorithmic}[1]
\STATE \COMMENT{--------------------------------------------}
\STATE {\bf function updateDictionary}($\bs{D}^{i,j},\bs{A}^{i,j},\bs{B}^{i,j}$)
\REPEAT
%\COMMENT{Update each dictionary element:}
\FOR{$j = 1$ to $k$}
\STATE
$
\boldsymbol{u}_j
\gets
\frac{
	\boldsymbol{b}_j
	-
	 \sum_{k \not = j} \boldsymbol{d}_k  a_{jk}
}
{
	a_{jj}
}
$
\label{as:dict_element_compute}
%\\
%&
%\algshade{
\\
\algshade{
\STATE
%\begin{align*}
%\begin{align*}
$
\boldsymbol{v}_j
\gets
Prox_{\lambda_j ||.||_1}(\boldsymbol{u}_j)
=
sgn(\boldsymbol{u}_j) (|\boldsymbol{u}_j| - \lambda_j)_{+},
$
\COMMENT{link sparsity}
%$\COMMENT{$\lambda_j$ tuned to get $\beta_d$ non-zeros in $\boldsymbol{v}_j$}
\label{as:sparse_elements}
%}
%\\
%&
\\
%\algshade{

\STATE
$
\boldsymbol{w}_j
\gets
\boldsymbol{v}_j
\left(
	1
	-
	\frac{\lambda_g}{||\boldsymbol{v}_j||_2}
\right)_{+}
$
\COMMENT{group (node) sparsity}
}
\label{as:kill_elements}
\\
\STATE
$
\boldsymbol{d}_j
\gets
\frac{
	\boldsymbol{w}_j
}
{
	\max(1, ||\boldsymbol{w}_j||_2)
}	
$
\label{as:dict_element_normalize}
\ENDFOR
\UNTIL{\textbf{convergence}}
\RETURN $\bs{D}^{i,j},\bs{A}^{i,j},\bs{B}^{i,j}$
%\label{as:dict_update_until_converge}
\end{algorithmic}
\label{alg:ODSDL}
\end{algorithm}
\end{small}
%\vspace{-0.05in}


==> sec_alg_bullet_points.tex <==
\begin{enumerate}
\item  initialize all W, D and C (e.g., randomly)
\item for each new sample $x_t$ with label $y_t$ (or minibatch):
\begin{enumerate}
\item for each layer i, from 1 to k: 
\begin{enumerate}
\item encode the sample at hidden layer  via proximal method combining 4 losses: reconstructive losses from this layer to the input, from this layer to the previous, and from the next layer to this one; predictive - from this layer to the label y: and from this 
\begin{eqnarray} \min_{c^i}  \sum_{j \in \{0,i-1\}}
  l^r ( {\bf D^{ij}},{\bf c^i}|{\bf c^j}) + \nonumber  
    l^r ( {\bf D^{i+1 i}},{\bf c^{i+1 } }|{\bf c^i}) + \nonumber \\
  \alpha    
  l^p ({\bf W^{i k+1}}, {\bf y}|{\bf c^i}) +  \lambda_{c}  ||\boldsymbol{c^i}||_1. ~~~~~~~
  \end{eqnarray}
  \item  update dictionary $D^{i i-1}$ from layer i to layer i-1 by iterating till convergence over its columns  \item if $i > 1$, update dictionary $D^{i 0}$ from layer i to layer 0 (x) by iterating till convergence over its $p$ columns: ${\bs D}^{i i-1} = $
\begin{eqnarray} \arg \min_{D}     \frac{1}{T} \sum_{t=1}^T \frac{1}{2} || \bs{c_t^{i-1}} - \bs{D} \bs{c_t^i} ||_2^2 +  \lambda_D ||\bs{D}||_1 + \nonumber \\
\gamma \sum_{j=1}^p  ||\bs{d_j}||_1 ~~~~~
  \end{eqnarray}
  \item if $i>1$ then same step as above is repeated for another dictionary, ${\bs D}^{i 0}$ whose links point from layer i codes to data (level 0).
\item  update predictive weights ${\bs W}$ from layer i to class label y (layer k+1),   fitting multinomial regression from $c^i$ to y, until convergence, using  gradient  descent. 
\end{enumerate}
\end{enumerate}
\end{enumerate}


==> sec_algorithm.tex <==
\section{Multinomial Regression}
Let $y_{ij}$ be an indicator for class $i$ for sample $j$. Let $c_j$ be the $j^{th}$ code learned from the dictionary learning which is the input features to our multinomial regression. Let $w_i$ be the weight vector learned for class $i$ with $W=[w_1,\ldots,w_{k-1}]$ and $k$ being the number of classes.  Then we model the likelihoods as
\[
P(y_{ij}=1 | c_i, W)=\frac{\exp{(w_i^Tc_j)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}, i=1,\ldots,k-1
\]
and
\[
P(y_{ij}=1 | c_j, W)=\frac{1}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}, i=k
\]
Then the log-likelihood function is
\[
\begin{array}{ll}
l(W)&=\displaystyle\sum_{j=1}^{n}{\log{P(y_j | c_j, W)}}\\
&=\displaystyle\sum_{j=1}^{n}{\log{\Big(\displaystyle\prod_{i=1}^k{P(y_{ij}=1 | c_j, W)^{y_{ij}}}\Big)}}\\
&=\displaystyle\sum_{j=1}^{n}{\log{\Big(\Big(\displaystyle\prod_{i=1}^{k-1}{\Big(\frac{\exp{(w_i^Tc_j)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}\Big)^{y_{ij}}\Big(\frac{1}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}\Big)^{y_{kj}}}}\Big)}\\
&=\displaystyle\sum_{j=1}^{n}{\Big(\displaystyle\sum_{i=1}^{k-1}{y_{ij}(w_i^Tc_j-\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})})}-y_{kj}\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})}}}\Big)}\\
&=\displaystyle\sum_{j=1}^{n}{\Big(\displaystyle\sum_{i=1}^{k-1}{y_{ij}(w_i^Tc_j)-\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})})}}\Big)}

\end{array}
\]

Then the full supervised dictionary learning problem minimizes the following objective

\[
F(c)=\displaystyle\sum_{j=1}^{n}{\Big(\|Dc_j-x_j\|_2^2-\displaystyle\sum_{i=1}^{k-1}{y_{ij}(w_i^Tc_j)+\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})})}}\Big)}
\]

In terms of the code $c$ we can minimize $n$ codes in parallel and concentrate on minimizing the function
\[
f(c)=\|Dc-x\|_2^2-\displaystyle\sum_{i=1}^{k-1}{y_{i}(w_i^Tc)+\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)})})}}
\]
where we've removed the index $j$ that represented sample $j$.  We first compute the gradient of $f(c)$ with respect to $c_a$ (the $a^{th}$ component of vector $c$).
\[
\frac{\partial f(c)}{\partial c_a} = (D^T(Dc-x))_a - \displaystyle\sum_{i=1}^{k-1}y_iw_{ia} + \displaystyle\sum_{i=1}^{k-1}{w_{ia}\Big(\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)}}}\Big)}
\]

In matrix vector notation, we have
\[
\nabla f = D^T(Dc-x) -Wy + W\Big(\frac{\exp{(W^Tc)}}{1+\textbf{1}^T\exp{(W^Tc)}}\Big)
\]
where the exponential and division functions on the right-hand side are component-wise. We next want to show that $\nabla f$ is Lipschitz continuous.  In order to do this, we will show that $\nabla^2 f \preceq LI$ for some $L>0$.  First, we compute the hessian of $f(c)$
\[
\begin{array}{ll}
\frac{\partial^2 f(c)}{\partial c_a\partial c_b} &= (D^TD)_{ab} + \displaystyle\sum_{i=1}^{k-1}{w_{ia}\Big(w_{ib}\Big(\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{w_l^Tc}}\Big)-\frac{\exp{(w_i^Tc)}\sum_{l=1}^{k-1}{w_{lb}\exp{(w_l^Tc)}}}{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)}})^2}\Big)}\\
&=(D^TD)_{ab} + \displaystyle\sum_{i=1}^{k-1}{w_{ia}w_{ib}\Big(\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)}}}\Big)}-\displaystyle\sum_{i=1}^{k-1}{\displaystyle\sum_{l=1}^{k-1}{w_{ia}w_{lb}\Big(\frac{\exp{(w_i^Tc)}\exp{(w_l^Tc)}}{(1+\sum_{m=1}^{k-1}{\exp{(w_m^Tc)}})^2}  \Big)}}
\end{array}
\]
We now write the hessian in matrix vector form.  Let $d\in\Re^{k-1}$ be a vector with
\[
\begin{array}{lll}
d_i&=\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{\exp{(w_i^Tc)}}}&=\frac{\exp{(w_i^Tc)}}{1+\exp{(w_i^Tc)}+\sum_{l=1,l\ne i}^{k-1}{w_l^Tc}}\\
&\leq \frac{\exp{(w_i^Tc)}}{1+\exp{(w_i^Tc)}}& \leq 1
\end{array}
\]

Then we can write the hessian as
\[
\nabla^2 f = D^TD + W\mbox{diag}(d)W^T + (Wd)(Wd)^T
\]

In order to bound the largest eigenvalue of the Hessian, we bound the three pieces separately so that
\[
L \geq \lambda_{\max}(D^TD) + \lambda_{\max}(W\mbox{diag}(d)W^T) + \lambda_{\max}((Wd)(Wd)^T)
\]

We have more work to do since $d$ is a function of the variable $c$. We have
\[
\lambda_{\max}(W\mbox{diag}(d)W^T)\leq\max_{i}(d_{i})\lambda_{\max}(WW^T)\leq\lambda_{\max}(WW^T)
\]
using the bound on $d_i$ above, and
\[
\lambda_{\max}((Wd)(Wd)^T) \leq d^T(WW^T)d \leq \|d\|_2^2\lambda_{\max}(WW^T)\leq(k-1)\lambda_{\max}(WW^T)
\]
since $d_i^2 \leq 1$. Finally, the Hessian is bounded
\[
L \geq \lambda_{\max}(D^TD) + \lambda_{\max}(WW^T) + (k-1)\lambda_{\max}(WW^T)=\lambda_{\max}(D^TD) + k\lambda_{\max}(WW^T)
\]
 


==> sec_approach.tex <==
\section{Multinomial Regression}
Let $y_{ij}$ be an indicator for class $i$ for sample $j$. Let $c_j$ be the $j^{th}$ code learned from the dictionary learning which is the input features to our multinomial regression. Let $w_i$ be the weight vector learned for class $i$ with $W=[w_1,\ldots,w_{k-1}]$ and $k$ being the number of classes.  Then we model the likelihoods as
\[
P(y_{ij}=1 | c_i, W)=\frac{\exp{(w_i^Tc_j)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}, i=1,\ldots,k-1
\]
and
\[
P(y_{ij}=1 | c_j, W)=\frac{1}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}, i=k
\]
Then the log-likelihood function is
\[
\begin{array}{ll}
l(W)&=\displaystyle\sum_{j=1}^{n}{\log{P(y_j | c_j, W)}}\\
&=\displaystyle\sum_{j=1}^{n}{\log{\Big(\displaystyle\prod_{i=1}^k{P(y_{ij}=1 | c_j, W)^{y_{ij}}}\Big)}}\\
&=\displaystyle\sum_{j=1}^{n}{\log{\Big(\Big(\displaystyle\prod_{i=1}^{k-1}{\Big(\frac{\exp{(w_i^Tc_j)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}\Big)^{y_{ij}}\Big(\frac{1}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)}}}\Big)^{y_{kj}}}}\Big)}\\
&=\displaystyle\sum_{j=1}^{n}{\Big(\displaystyle\sum_{i=1}^{k-1}{y_{ij}(w_i^Tc_j-\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})})}-y_{kj}\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})}}}\Big)}\\
&=\displaystyle\sum_{j=1}^{n}{\Big(\displaystyle\sum_{i=1}^{k-1}{y_{ij}(w_i^Tc_j)-\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})})}}\Big)}

\end{array}
\]

Then the full supervised dictionary learning problem minimizes the following objective

\[
F(c)=\displaystyle\sum_{j=1}^{n}{\Big(\|Dc_j-x_j\|_2^2-\displaystyle\sum_{i=1}^{k-1}{y_{ij}(w_i^Tc_j)+\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc_j)})})}}\Big)}
\]

In terms of the code $c$ we can minimize $n$ codes in parallel and concentrate on minimizing the function
\[
f(c)=\|Dc-x\|_2^2-\displaystyle\sum_{i=1}^{k-1}{y_{i}(w_i^Tc)+\log{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)})})}}
\]
where we've removed the index $j$ that represented sample $j$.  We first compute the gradient of $f(c)$ with respect to $c_a$ (the $a^{th}$ component of vector $c$).
\[
\frac{\partial f(c)}{\partial c_a} = (D^T(Dc-x))_a - \displaystyle\sum_{i=1}^{k-1}y_iw_{ia} + \displaystyle\sum_{i=1}^{k-1}{w_{ia}\Big(\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)}}}\Big)}
\]

In matrix vector notation, we have
\[
\nabla f = D^T(Dc-x) -Wy + W\Big(\frac{\exp{(W^Tc)}}{1+\textbf{1}^T\exp{(W^Tc)}}\Big)
\]
where the exponential and division functions on the right-hand side are component-wise. We next want to show that $\nabla f$ is Lipschitz continuous.  In order to do this, we will show that $\nabla^2 f \preceq LI$ for some $L>0$.  First, we compute the hessian of $f(c)$
\[
\begin{array}{ll}
\frac{\partial^2 f(c)}{\partial c_a\partial c_b} &= (D^TD)_{ab} + \displaystyle\sum_{i=1}^{k-1}{w_{ia}\Big(w_{ib}\Big(\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{w_l^Tc}}\Big)-\frac{\exp{(w_i^Tc)}\sum_{l=1}^{k-1}{w_{lb}\exp{(w_l^Tc)}}}{(1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)}})^2}\Big)}\\
&=(D^TD)_{ab} + \displaystyle\sum_{i=1}^{k-1}{w_{ia}w_{ib}\Big(\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{\exp{(w_l^Tc)}}}\Big)}-\displaystyle\sum_{i=1}^{k-1}{\displaystyle\sum_{l=1}^{k-1}{w_{ia}w_{lb}\Big(\frac{\exp{(w_i^Tc)}\exp{(w_l^Tc)}}{(1+\sum_{m=1}^{k-1}{\exp{(w_m^Tc)}})^2}  \Big)}}
\end{array}
\]
We now write the hessian in matrix vector form.  Let $d\in\Re^{k-1}$ be a vector with
\[
\begin{array}{lll}
d_i&=\frac{\exp{(w_i^Tc)}}{1+\sum_{l=1}^{k-1}{\exp{(w_i^Tc)}}}&=\frac{\exp{(w_i^Tc)}}{1+\exp{(w_i^Tc)}+\sum_{l=1,l\ne i}^{k-1}{w_l^Tc}}\\
&\leq \frac{\exp{(w_i^Tc)}}{1+\exp{(w_i^Tc)}}& \leq 1
\end{array}
\]

Then we can write the hessian as
\[
\nabla^2 f = D^TD + W\mbox{diag}(d)W^T + (Wd)(Wd)^T
\]

In order to bound the largest eigenvalue of the hessian, we bound the three pieces separately so that
\[
L \geq \lambda_{\max}(D^TD) + \lambda_{\max}(W\mbox{diag}(d)W^T) + \lambda_{\max}((Wd)(Wd)^T)
\]

We have more work to do since $d$ is a function of the variable $c$. We have
\[
\lambda_{\max}(W\mbox{diag}(d)W^T)\leq\max_{i}(d_{i})\lambda_{\max}(WW^T)\leq\lambda_{\max}(WW^T)
\]
using the bound on $d_i$ above, and
\[
\lambda_{\max}((Wd)(Wd)^T) \leq d^T(WW^T)d \leq \|d\|_2^2\lambda_{\max}(WW^T)\leq(k-1)\lambda_{\max}(WW^T)
\]
since $d_i^2 \leq 1$. Finally, the hessian is bounded
\[
L \geq \lambda_{\max}(D^TD) + \lambda_{\max}(WW^T) + (k-1)\lambda_{\max}(WW^T)=\lambda_{\max}(D^TD) + k\lambda_{\max}(WW^T)
\]

==> sec_background.tex <==
\vspace{-0.015in}
\section{Background on Dictionary Learning}
\label{sec:background_dictionary_learning}
\vspace{-0.01in}
% standard dictionary learning
\subsection{Offline learning}
Traditional off-line {\em dictionary learning}  \cite{olshausen1997sparse,aharon2006k,lee2006efficient}, also known as {\em sparse coding},  aims at  finding a {\em dictionary} $\bs{D} \in \mathbb{R}^{m \times k}$,
 which allows for an accurate  encoding of each sample in the training data set  $\bs{X} = \{ \bs{x}_1, \cdots, \bs{x}_n \in \mathbb{R}^m \}$ by a linear combinations of a {\em relatively small}
 subset  of
{\em  dictionary elements}   $\bs{D} = \{ \bs{d}_1, \cdots, \bs{d}_k \in \mathbb{R}^m \}$, which is  represented, for each $\bs{x}_i$,  by its {\em sparse code} (i.e., a vector with a few nonzeros) $\bs{c}_i \in \mathbb{R}^k$. In order to prevent the dictionary entries from growing arbitrarily large, it is common to impose on them a norm constraint \cite{mairal2009online,mairal2010online}, i.e. keep
  the columns of $\bs{D}$ within the convex set  $\mathcal{C}= \{\boldsymbol{D} \in \mathbb{R}^{m \times k} $ $~~s.t.~~ \forall j~ \boldsymbol{d}^T_j \boldsymbol{u}_j \leq 1 \}$.
  Denoting the set of codes as $\bs{C} = \{ \bs{c}_1, \cdots, \bs{c}_n \in \mathbb{R}^k \}$, the (offline) dictionary learning  is formulated as   minimization of the total {\em reconstructive loss} objective $f_n\bs{D},\bs{C}|\bs{X})$
over $\bs{D}$ and $\bs{C}$:
\begin{eqnarray}
\label{eqn:dic_learn_objective}
\min_{\bs{D \in \mathcal{C}},\bs{C}} f_n(\bs{D},\bs{C}|\bs{X})
= \min_{\bs{D}}\frac{1}{n} \sum_{i=1}^n l(\bs{D}|\bs{x}_i)
\vspace{-0.05in}
\end{eqnarray}
where
\begin{eqnarray}
\label{eqn:lasso}
l(\bs{D}|\bs{x}) = \min_{\bs{c} \in \mathbb{R}^k} \frac{1}{2} || \bs{x} - \bs{D} \bs{c} ||_2^2 + \lambda_{c} || \bs{c} ||_1.
\vspace{-0.05in}
\end{eqnarray}
 The first term is the representation error, and the second term
is the $l_1$-regularization which enforces  the {\em codes}  $\bs{c}_i$
 to be sparse. The joint minimization of $L^R_n(D,C)$ with respect to the dictionary and codes is non-convex, and commonly used approach
is to use an alternating minimization over the codes and the dictionary.
	
\subsection{Online learning}
However, the classical dictionary learning does not scale to very large datasets; moreover, it is not immediately applicable to online learning from a continuous stream of data.
The {\em online dictionary learning (ODL)} method proposed by \cite{mairal2009online} overcomes both of these limitations, and serves as a basis for our proposed approach,
presented in \algoref{alg:neurogen_mairal} in the next section.
While the highlighted lines in \algoref{alg:neurogen_mairal} represent an adaptive, or ``neurogenetic'' extension of \mai previously proposed in \cite{garg2017},
the non-highlighted ones are common to both approaches, and are discussed first. The algorithms start with some dictionary $\boldsymbol{D}^{0}$,
 e.g. a randomly initialized one (other approaches include  using some of the inputs
as dictionary elements  \cite{mairal2009online,NIPS2009_3691}).
At each iteration $t$, both online approaches
consider the next input sample $\bs{x}_t$  (or a batch of samples), in   step \ref{as:input_data} %of \algoref{alg:neurogen_mairal}
and  compute its sparse code $\bs{\alpha}_t$
 by solving the LASSO \cite{tibshirani1996regression} problem (step \ref{as:sparse_coding}), % in \algoref{alg:neurogen_mairal}),
with respect to the current dictionary.
%\footnote{Since LASSO  typically assumes zero-mean, unit-variance columns of the ``data'' matrix \cite{tibshirani1996regression}, i.e. $\boldsymbol{D}^{(t-1)}$ in step 4 of \algoref{alg:neurogen_mairal},
% each dictionary element will be first normalized  to have zero mean and unit norm, as a preprocessing step before sparse coding}.
%In \algoref{alg:neurogen_mairal},
%  to simplify the notation.
Next,   \mai  computes the dictionary update,  $\bs{D}^{(t)}$ (denoted simply as  $\bs{D}$ in the algorithm), by optimizing  the {\em surrogate} objective function $\hat{f}_t(D)$,  similar to the
 original one  in eq. \eqnref{eqn:dic_learn_objective}, for  $n=t$, except for an important change: in eq. \eqnref{eqn:dic_learn_objective}, each code $\bs{\alpha}_i$ is computed using the {\em same} dictionary $\boldsymbol{D}$, while  the surrogate function keeps the codes
  $\bs{\alpha}_i$ %, \bs{\alpha}_2, \cdots, \bs{\alpha}_{t}$
   from the {\em previous} iterations, computed using the corresponding previous dictionaries  $\bs{D}^{(i)}$,  %,..., \bs{D}^{(t-1)}$,
 i.e.  {\em does not recompute} the  codes of  previously
  seen samples after each dictionary update.
  This speeds up the learning without worsening the (asymptotic) performance, since
 the surrogate objective   converges to the original one in \eqnref{eqn:dic_learn_objective}, under certain assumptions, including data stationarity  \cite{mairal2009online}.
  Note that, in order to prevent the dictionary entries from growing arbitrarily large, \cite{mairal2009online} impose the norm constraint, i.e. keep
  the columns of $\bs{D}$ within the convex set  $\mathcal{C}= \{\boldsymbol{D} \in \mathbb{R}^{m \times k} $ $~~s.t.~~ \forall j~ \boldsymbol{d}^T_j \boldsymbol{u}_j \leq 1 \}$.
   Then the dictionary  update step computes   $\bs{D}^{(t)} = \arg \min_{\boldsymbol{D} \in \mathcal{C}} \hat{f}_t(D)$, ignoring $l_1$-regularizer over the code which is fixed at this step,  i.e. it finds $\min_{\boldsymbol{D} \in \mathcal{C}} \frac{1}{t}
\sum_{i=1}^t \frac{1}{2} ||
\boldsymbol{x}_i - \boldsymbol{D} \boldsymbol{\alpha}_i
||_2^2  $, which is equivalent to  finding
\vspace{-0.05in}
\begin{eqnarray}
\label{eqn:optimize_dict_obj}
  \min_{\boldsymbol{D} \in \mathcal{C}}
\frac{1}{2}
Tr(\boldsymbol{D}^T\boldsymbol{D}\boldsymbol{A}) - Tr(\boldsymbol{D}^T\boldsymbol{B}),
%\vspace{-0.02in}
\vspace{-0.05in}
\end{eqnarray}
  where $\bs{A} = \sum_{i=1}^t \boldsymbol{\alpha}_i \boldsymbol{\alpha}_i^T$ and $\bs{B} = \sum_{i=1}^t \boldsymbol{x}_i \boldsymbol{\alpha}_i^T$ are the ``bookkeeping''
  matrices (we also call them ``memories'' of the model), compactly representing the input samples and encoding history.
   At each iteration, once the new input sample $\boldsymbol{x}_i $ is encoded,
    the matrices are updated as $\boldsymbol{A} \gets \boldsymbol{A} + \boldsymbol{\alpha}_t \boldsymbol{\alpha}_t^T$ and $\boldsymbol{B}
\gets
\boldsymbol{B} + \boldsymbol{x}_t \boldsymbol{\alpha}_t^T$ (see the step \ref{as:memory_update}  of \algoref{alg:neurogen_mairal}).
In \cite{mairal2009online}, a \emph{block coordinate descent} is used to optimize
 the convex objective
 %\footnote{Convexity follows since  the Hessian $\bs{A}$ is guaranteed to be positive semi-definite since it is the empirical covariance  of the codes.}
 in eq. \ref{eqn:optimize_dict_obj}; it iterates over the dictionary elements in a fixed sequence, until convergence, optimizing each while
 keeping the others fixed as shown in eq. \eqnref{eqn:dict_update} (steps \ref{as:dict_element_compute} and \ref{as:dict_element_normalize} in \algoref{alg:neurogen_mairal}, except that, in our approach,
$\boldsymbol{u}_j$ is transformed into $\boldsymbol{w}_j$   to impose an additional regularizer before computing step \ref{as:dict_element_normalize}).
\vspace{-0.05in}
\begin{align}
\label{eqn:dict_update}
&
%\underbrace{
\boldsymbol{u}_j
\gets
\frac{
	\boldsymbol{b}_j
	-
	 \sum_{k \not = j} \boldsymbol{d}_k  a_{jk}
}
{
	a_{jj}
}
%}_{\text{minimize the least square error}}
;\ \ \
%\underbrace{
\boldsymbol{d}_j
\gets
\frac{
	\boldsymbol{u}_j
}
{
	\max(1, ||\boldsymbol{u}_j||_2)
}
%}_{\text{norm less than one~(the convex constraint $\bs{D} \in \mathcal{C}$)}}
%\vspace{-0.02in}
\vspace{-0.05in}
\end{align}

%
In \cite{garg2017}, sparsity regularizer is also imposed on  dictionary elements (step 15 in \algoref{alg:neurogen_mairal}), i.e. the  objective in eq. \eqnref{eqn:optimize_dict_obj} is replaced with the following one:
\begin{equation}
\label{eqn:optimize_dict_obj_sparse}
\min_{\boldsymbol{D} \in \mathcal{C}}
\frac{1}{t}
\sum_{i=1}^t
\frac{1}{2}
||
\boldsymbol{x}_i - \boldsymbol{D} \boldsymbol{\alpha}_i
||_2^2
+
\sum_j
\lambda_j
||
\boldsymbol{d}_j
||_1.
\vspace{-0.02in}
\end{equation}

\subsection{Neurogenic Online Dictionary Learning}
\label{sec:mairal_neurogen}
In \cite{garg2017}, the online dictionary learning  designed for stationary input distributions, was extended to a more adaptive framework capable of  handling nonstationary data effectively, and
learning to represent new types of data without forgetting how to represent the old ones.

Towards this end, we  propose a novel algorithm, called Neurogenetic Online Dictionary Learning (see \algoref{alg:neurogen_mairal}), which can flexibly extend and reduce a dictionary in response to the changes
in an input distribution, and possibly to the inherent representation complexity of the data. The main changes, as compared to the non-adaptive, fixed-dictionary-size algorithm of \cite{mairal2009online}, are highlighted in \algoref{alg:neurogen_mairal}; the two parts involve (1) neurogenesis, i.e. the addition of dictionary elements (hidden units, or ``neurons'') and  (2) the death
of old and/or new elements which are ``less useful'' than other elements for the task of data reconstruction.

At each iteration in \algoref{alg:neurogen_mairal}, the next batch of samples is received and the corresponding codes, in the dictionary, are computed; next, we add  $k_{n}$  new dictionary elements sampled at random from $\mathbb{R}^m$
(i.e., $k_{n}$ random linear projections of the input sample). The choice of the parameter $k_{n}$ is important; one approach is to tune it  (e.g., by cross-validation), while another is
to adjust it dynamically, based on the dictionary performance: e.g., if the environment is changing, the old dictionary may not be able to represent the new input well, leading to decline
in the representation accuracy, which  triggers neurogenesis. Herein,  we  use as the performance measure the Pearson correlation between a new sample and
its representation in the current dictionary $r(\bs{x}_t,\bs{D}^{(t-1)}\bs{\alpha}_	t)$, i.e. denoted as $p_c(\boldsymbol{x}_t, \boldsymbol{D}^{(t-1)}, \boldsymbol{\alpha}_t)$~(for a batch of data, the average over $p_c(.)$ is taken). If it drops below a certain pre-specified threshold  $\gamma$ (where $0 \ll \gamma \leq 1$), the neurogenesis is triggered (the step \ref{as:condition_neurogenesis}). The number $k_{n}$  of new dictionary elements  is proportional to the
error   $1-p_c(\cdot)$, so that worse performance will trigger more neurogenesis, and vice versa; the maximum number of new elements is bounded by $c_k$ (the step \ref{as:num_new_neurons}).
% %\vspace{-6mm}
%\begin{align}
%k_{n} =
%\begin{cases}
%0  \text{if } p_c(\boldsymbol{x}_1, \cdots, \boldsymbol{x}_b, \boldsymbol{D}, \boldsymbol{\alpha}_1,  \cdots, \boldsymbol{\alpha}_b) \leq \gamma\\
%(1-c(\boldsymbol{x}_1, \cdots, \boldsymbol{x}_b, \boldsymbol{D}, \boldsymbol{\alpha}_1,  \cdots, \boldsymbol{\alpha}_b)) c_k otherwise\\
%\end{cases},
%\label{eqn:conditional_birth}
%\vspace{-6.5mm}
%\end{align}
%where $0 \ll \gamma \leq 1$ is a performance threshold for triggering neurogenesis,
%and $c_k$ is the upper limit on the value of $k_{n}$. These parameters need minimal tuning.
We refer to this approach as \emph{conditional neurogenesis} as it involves the \emph{conditional birth} of new elements.
Next, $k_n$ random elements are generated and added to the current dictionary  (the step \ref{as:init_new_elements}),
and the memory matrices $\bs{A}, \bs{B}$ are updated, respectively, to account for larger dictionary  (the step \ref{as:memory_increase}).
Finally, the sparse code is recomputed for $\bs{x}_t$~(or, all the samples in the current batch) with respect to the extended dictionary (the step \ref{as:recompute_sparse_code}).

\begin{small}
\input{./sec_our_algo_pseudo_code}
\end{small}

The next step is the dictionary update, which uses block-coordinate descent, with the following objective function:
% to eq. \eqnref{eqn:optimize_dict_obj}:
%
%
\vspace{-0.01in}
\begin{small}
\begin{equation}
\label{eqn:optimize_dict_obj_group_sparse}
%\bs{D}^{(t)}
%\!
%=
%\!
%\arg
\min_{\boldsymbol{D} \in \mathcal{C}}
%\hat{f}_t(D);\
%\hat{f}_t(D)
%\!
%=
%\!
%\underbrace{
\frac{1}{t}
\sum_{i=1}^t
\frac{1}{2}
||
\boldsymbol{x}_i - \boldsymbol{D} \boldsymbol{\alpha}_i
||_2^2
%}_{\text{reconstruction error}}
+
%\underbrace{
\lambda_g
\sum_j
||\boldsymbol{d}_j||_2
%}_{\text{$l_{1}/l_2$ group sparsity}}
+
%\underbrace{
\sum_j
\lambda_j
||
\boldsymbol{d}_j
||_1.
%}_{\text{sparse elements~(optional)}}
\vspace{-0.01in}
\end{equation}
\end{small}
%
\noindent The first term is the standard reconstruction error, as before. The second term, $l_1/l_2$-regularization, promotes group sparsity over the dictionary entries, where each
group corresponds to a column, i.e. a dictionary element. The group-sparsity \cite{yuan2006model} regularizer causes some columns in $\boldsymbol{D}$  to be set to zero (i.e. the  columns
 less useful for accurate data representation), thus effectively eliminating
the corresponding dictionary elements from the dictionary (``killing'' the corresponding hidden units).
As mentioned previously, \cite{NIPS2009_3691} used the $l_1/l_2$-regularizer in dictionary learning, though not in online setting, and without neurogenesis.

Finally, the third term imposes $l_1$-regularization on dictionary elements thus promoting sparse dictionary, besides the sparse coding. Introducing sparsity in dictionary elements, corresponding
to the sparse connectivity of hidden units in the neural net representation of a dictionary, is motivated by both their biological plausibility (neuronal connectivity tends to be rather sparse
in multiple brain networks), and by the computational advantages this extra regularization can provide, as we observe later in experiments section~(\secref{sec:experiments}).

As in the original algorithm of \cite{mairal2009online}, the above objective is optimized by the block-coordinate descent,  where each block of variables corresponds to a dictionary element,
i.e., a column in $\boldsymbol{D}$; the loop in steps \ref{as:dict_update_repeat}-\ref{as:dict_update_until_converge} of the \algoref{alg:neurogen_mairal} iterates until convergence, defined by the magnitude of change between the two successive versions of the dictionary
falling below some threshold. For each column update, the first and the last steps (the steps \ref{as:dict_element_compute} and \ref{as:dict_element_normalize}) are the same as in the original method of \cite{mairal2009online},
while the two intermediate steps (the steps \ref{as:sparse_elements} and \ref{as:kill_elements}) are implementing additional regularization.
Both steps \ref{as:sparse_elements} and \ref{as:kill_elements} (sparsity and group sparsity regularization) are implemented using the standard proximal operators
 as described in \cite{jenatton2011proximal}. Note that we actually use as input the desired number of non-zeros, and determine the corresponding sparsity parameter
%$\lambda_g$,
$\lambda_c$ and $\lambda_j$
 using a binary search procedure. %~(see Appendix).
Overall, \emph{the key features of our algorithm is the interplay of both the (conditional) birth and (group-sparsity) death of dictionary elements in an online setting.}








==> sec_formulation_ODSDL.tex <==
\vspace{-0.015in}
\section{Problem Formulation}
\label{sec:formulation}
Similarly to deep learning objective, our motivation here is to learn a hierarchy of representations, or feature vectors, which would hopefully be able to capture hierarchical structures in data, from most detailed to most abstract. We will focus later on an {\em online, lifelong learning}, where the data continue arriving in mini-batches; however, we will first start with the {\em offline} formulation.

\noindent {\bf Network model.} As usual, features at different level of abstraction are represented by layers of hidden variables (units, or neurons). However, we assume a more general connectivity than
standard feedforward neural nets: namely, we allow for both forward and
backward links from each layer to any other layer, including the input layer
and the output layer. The variables in the same layer, however, are disconnected (see Figure 1). While such architecture can potentially have too many parameters, we will apply sparsity regularizer which will trim the architecture adaptively, online, choosing  an appropriate, data-driven combination of forward and backward links, instead of engineering the architecture manually as it was previously done in  (LadderNet, ResNet, DenseNet, HighwayNets and so on). Our approach can be also viewed as a mix of feedforward neural nets with sparse coding (dictionary learning) represented by backward links. In the online formulation presented later, we will also include architecture adaptation not only at the link, but at the node level, as proposed earlier in  (Garg2017, NonparamNets), where hidden variables can be added and deleted depending on the performance of the model in online setting; node deletion is implemented via group sparsity.


\noindent {\bf Notation.} Let $\bs{X} = \{ \bs{x}_1, \cdots, \bs{x}_n \in \mathbb{R}^m \}$ represent input samples and let  $\bs{Y}= \{y_1, \cdots, y_n \}$ represent the corresponding class labels. We denote by $\bs{c^j}$ hidden variables, or ''codes'', at layer $j$, $j=0,...,k$, and  by $\bs {W^j}$ the weight matrix associated with connections from layer $j$ to layer $j+1$, where each column corresponds to an output variable at the next level $j+1$, and each row corresponds to a variable in the hidden layer $j$, or in case of j=0, input layer; in case of the last layer pointing to the output variable $y$, the matrix is just a column vector. Next, we use $\bs {D^j}$,  $j=1,...,k$, to denote the backward link weights (''dictionary elements'' as in sparse coding) from layer $j$ to the input layer (layer 0).


\subsection{Offline learning}
We will first consider a classical offline learning problem:
 given a training data set $(\bs{X},Y)$, estimate model parameters y
 minimizing the cost function associated with our network model.
 Our cost function, however, differs from traditional feedforward net cost
 function in following two aspects. First, we explicitly optimize not just the link weights, but also the hidden unit activations, or codes in sparse coding terminology (or auxiliary variables of (Carreira-Perpinian)). This  allows for a problem decomposition into multiple convex  subproblems easily solved via alternating minimization procedure; this is the second major difference in parameter optimization, as opposed to traditional backpropagation via SGD. Our cost function is a weighted sum of local loss
 functions associated with sets of either forward or backward   links connecting each hidden layer to another one, above or below it, as well as sparsity and group sparsity regularizer on networks links, allowing for both
 link and node deletion. (Later we describe an extension of this approach to an  online architecture adaptation algorithm which combines both deletion and addition of links and nodes in response to input data, similar in spirit to (Garg, NonparamNets)). 
 
\noindent {\bf Supervised dictionary learning: single hidden-layer reconstructive-predictive network.} Let us first consider a very simple single-hidden layer architecture and the following  objective, we refer to as  ''supervised dictionary learning'' (though a bit different from Mairal, etc.), which extends the standard dictionary learning (sparse coding) objective (see Appendix, section \ref{sec:background_dictionary_learning}) to a include both the {\em reconstructive loss} ${l}_r ({\bf D}, {\bf c}|{\bf x})$, i.e. the loss associated with reconstructing a sample ${\bf x} \in \mathbb{R}^m$ given an $m \times p$ dictionary ${\bf D}$ and a sparse code ${\bf c} \in \mathbb{R}^p$,
 and {\em predictive loss}  ${l}_p ( {\bf W}, {\bf c}|{\bf y})$ of predicting  a set of $r$ labels ${\bf y}$ given the sparse code and a $p \times r$ parameter matrix {\bf W} of $r$ classifiers. The loss functions 
 above will correspond to GLM regression losses, i.e. those for linear, logistic or multinomial regression, depending on the type of the variables.
 For example, the reconstructive loss is typically sum-squared loss (assuming 
 linear regression from codes to the data), i.e. ${l}_r ({\bf D}, {\bf c}|{\bf x}) = ||{\bf x} - {\bf D} {\bf c}||_2^2$, while {\em predictive losses are typically multinomial/cross-entropy (associated with the class label) or logistic (e.g., associated with binary hidden units)}.
 \begin{eqnarray}
\label{eqn:objective_supervised_dict}
\min_{\bs{D},\bs{W}} f_n(\bs{D},\bs{W})
= \min_{\bs{D},\bs{W}}\frac{1}{n} \sum_{i=1}^n l(\bs{D}, \bs{W}|\bs{x}_i),
\end{eqnarray}
where  $ l(\bs{D}, \bs{W}|\bs{x}) =$
 \begin{eqnarray}
\label{eqn:SDL_loss}
 \min_{{\bf c} \in \mathbb{R}^p} l^r ( {\bf D}, {\bf c}|{\bf x}) + \alpha l^p ({\bf W}, {\bf c}|{\bf y}) +  \lambda_{c}||\boldsymbol{c}||_1 + \\ \lambda_W ||\boldsymbol{W}||_1 + \lambda_D ||\boldsymbol{D}||_1 + \gamma \sum_{j=1}^p  ||\boldsymbol{d_j}||_1.
%\vspace{-0.13in}
\end{eqnarray}
Parameter $\alpha$ controls the trade-off between the predictive and reconstructive losses, and the last four terms are:
$l_1$-regularization enforcing code sparsity, weight link sparsity, both for predictive weights ${\bf W}$ and reconstructive weights, or dictionary ${\bf D}$. Finally, the last term is the group sparsity over the dictionary columns ${\bf{d}_j}$; group sparsity enforces setting to zero, or eliminate if needed the whole column, i.e. all links adjacent to a particular hidden node, which leads to node deletion.   . 

The problem in the eq. \ref{eqn:objective_supervised_dict} can be also written as a joint optimization over $\bs D$, $\bs W$, and code matrix $\bs C= \{{\bs c}_i\}$, given the data matrix ${\bs X}$ and the corresponding label matrix ${\bs Y}$:
 \begin{eqnarray}
 \min_{\bs{D},\bs{W},\bs{C}}\frac{1}{n} \sum_{i=1}^n  L^r ( {\bf D}, {\bs C}|{\bs X}) + \alpha L^p ({\bf W}, {\bs C}|{\bs Y}) +  \\ \lambda_{c}||{\bs C}||_1 +  \lambda_W ||\boldsymbol{W}||_1 + \lambda_D ||\boldsymbol{D}||_1 + \gamma \sum_{j=1}^p  ||\boldsymbol{d_j}||_1,
 \end{eqnarray}
where $L^r ( {\bf D}, {\bs C}|{\bs X}) = \sum_{i=1}^n   l^r ( {\bf D}, {\bf c_i}|{\bf x_i})$ and   $L^p ( {\bf W}, {\bs C}|{\bs X}) = \sum_{i=1}^n   l^r ( {\bf D}, {\bf c_i}|{\bf x_i})$. Although the above joint minimization  is in general a nonconvex problem, a commonly used approach
is to use an alternating minimization, or block-coordinate, approach which alternates between optimizing over one of the sets ${\bs C}$, ${\bs D}$ and ${\bs W}$, while fixing the other two.

%\footnote{In our implementation,  an $L_2$-norm regularization was also added on all matrices $U,V,W$ with small regularization constants (0.01),
%effectively corresponding to assuming Gaussian priors on those matrices.}.

\noindent {\bf Deep predictive-reconstructive model: general case.} Next, we formulate a general objective for learning deep network architecture with both forward (predictive) and backward (reconstructive) links, as described before. We will change the notation now:  given an input ${\bs x} \in \mathbb{R}^m $ and an output (label) ${\bs y} \in \mathbb{R}^r$, $\bs{C} = \{\bs{c}^1 \in \mathbb{R}^{p_1}, \cdots, \bs{c}^k \in \mathbb{R}^{p_k} \}$ will denote
 the set of all codes (hidden node activations at layers from 1 to k, with $p_i$ hidden nodes in the $i$-th layer), $\bs{W} = \{ \bs{W}^{ij}| 0 \leq i \leq k, 1 \leq j \leq k+1\}$ will denote all forward link weights from a layer $i$ to layer $j$, and  $\bs{D} = \{ \bs{D}^{ij}, 1 \leq i \leq k, 0 \leq j \leq k-1\}$ will denote all backward link weights, from a layer $i$ to layer $j$. For convenience we also use the notation $\bs{c}_0 = \bs{x}$ and $\bs{c}_{k+1} = \bs{y}$.
\begin{eqnarray}
\label{eqn:objective}
\min_{\bs{D},\bs{W},\bs{C}} f_n(\bs{D},\bs{W},\bs{C}|\bs{X})
= \min_{\bs{D},\bs{W}}\frac{1}{n} \sum_{i=1}^n l(\bs{D}, \bs{W}|\bs{x}_i),
\end{eqnarray}
where
 \begin{eqnarray}
\label{eqn:SDL_loss}
  l(\bs{D}, \bs{W}|\bs{x}) = \min_{{\bf C}  } \sum_{i=1}^{k}  \sum_{j=0}^{i-1}    l^r ( {\bf D^{ij}}, {\bf c^i}|{\bf c^j}) + \nonumber \\
  \alpha \sum_{j=i+1}^{k+1}   l^p ({\bf W^{ij}}, {\bf c^j}|{\bf c^i}) +   \lambda_{c} ||\boldsymbol{c^i}||_1 +  \nonumber \\
  \lambda_W \sum_{j=i+1}^{k+1} ||\boldsymbol{W^{ij}}||_1 +  \lambda_D \sum_{j=0}^{i-1}  ||\boldsymbol{D^{ij}}||_1  + \gamma \sum_{s=1}^{s_{i}}  ||\boldsymbol{d^{ij}_s}||_1.
\end{eqnarray}
\noindent {\bf  Deep predictive-reconstructive model: special cases.} We will assume for now a  simplified version   of the above objective, where the
only forward connections allowed at any hidden layer are those going directly   to the output layer ${\bf y}$ (or ${\bf c^{k+1}}$, i.e.  ${\bf W}^{i {k+1}}$. The only backward connections are those going directly to the previous layer and all the way back to the input layer, i.e. ${\bf D}^{i {i-1}}$ and ${\bf D}^{i0}$. This architecture is known as {\em supervised deep dictionary learning} \citep{}[DeepDictionarypaper], with the corresponding loss function:
 \begin{eqnarray}
\label{eqn:SDL_loss_simple}
l(\bs{D}, \bs{W}|\bs{x}) = \min_{{\bf C}  } \sum_{i=1}^{k}
 \sum_{j \in \{0,i-1\}}
  l^r ( {\bf D^{ij}},{\bf c^i}|{\bf c^j}) + \nonumber \\
  \alpha    
  l^p ({\bf W^{i k+1}}, {\bf y}|{\bf c^i}) +
  \lambda_{c}  ||\boldsymbol{c^i}||_1 + \nonumber \\
  \lambda_W  ||\boldsymbol{W^{i {k+1}}}||_1 +
  \lambda_D    ||\boldsymbol{D^{i0}}||_1  +
  \gamma \sum_{s=1}^{s_{i}}  ||\boldsymbol{d^{i0}_s}||_1.
\end{eqnarray}



\subsection{Online learning}
However, offline (batch) learning performing optimization with respect to the potentially very large training dataset is not scalable.  Moreover, we would like to have an online approach which can adapt to a continuous stream of data in a lifelong learning setting. We build our approach on top of the  {\em online dictionary learning (ODL)} proposed in \cite{mairal2009online}. In \cite{mairal2009online}, we assume that, at $t$-th iteration of the algorithm, we obtain a sample $\bx_t$ (or a mini-batch of samples), which is first encoded into   ${\bf c}_t$ using the dictionary ${\bf D}_{t-1}$ from the previous iteration; then the dictionary update step is optimizing a following   {\em surrogate} objective function $\hat{f}_n(D)=$
\begin{eqnarray}
%\label{eqn:dic_learn_objective}
   \frac{1}{n} \sum_{t=1}^N \frac{1}{2} || \bs{x}_t - \bs{D} \bs{c}_t ||_2^2 + \lambda_{c} || \bs{c}_t ||_1,
\vspace{-0.05in}
\end{eqnarray}
where each 
\begin{eqnarray}
\bs{c}_t = \arg \min_{\bs{c}} \frac{1}{2} || \bs{x}_t - \bs{D_{t-1}} \bs{c} ||_2^2 + \lambda_{c} || \bs{c} ||_1.
\label{eq:Lasso}
\end{eqnarray}
The surrogate objective is similar to the
 original one  in eq. \eqnref{eqn:dic_learn_objective}, for  $n=N$, except for an important change: in eq. \eqnref{eqn:dic_learn_objective}, each code $\bs{c}_t$ is computed using the {\em same} dictionary $\boldsymbol{D}$, while  the surrogate function keeps the codes
  $\bs{c}_t$ %, \bs{\alpha}_2, \cdots, \bs{\alpha}_{t}$
   from the {\em previous} iterations, computed using the corresponding previous dictionaries,
 i.e.  {\em does not recompute} the  codes of  previously
  seen samples after each dictionary update.
  This speeds up the learning without worsening the (asymptotic) performance, since
 the surrogate objective   converges to the original one in \eqnref{eqn:dic_learn_objective}, under certain assumptions, including data stationarity  \cite{mairal2009online}.
 
 \noindent{\bf Online supervised dictionary learning.} Similarly to online dictionary learning, we assume that, given the new sample ${\bf x_t}$, we first encode it into ${\bf c_t}$ using current  dictionary as the solution to a LASSO problem, and then  formulate the surrogate objective for all  weights assuming the codes from the previous and current iterations being fixed: $\min_{\bs{D},\bs{W}} \hat{f}_n(\bs{D}, \bs{W})
=$
 \begin{eqnarray}
\label{eqn:sup_dl}
 \min_{\bs{D}, \bs{W}}\frac{1}{n} \sum_{t=1}^n  l^r ( {\bf D}, {\bf c}_t|{\bf x}_t) + \alpha l^p ({\bf W}, {\bf c}_t|{\bf y}_t) +  \nonumber \\
 \lambda_{c}||\boldsymbol{c}_t||_1 +   \lambda_W ||\boldsymbol{W}||_1 + \lambda_D ||\boldsymbol{D}||_1 + \gamma \sum_{j=1}^p  ||\boldsymbol{d_j}||_1, 
%\vspace{-0.05in}
\end{eqnarray}
where each code is computed as
\begin{eqnarray}
{\bs{c}}_t = \arg \min_{\bs{c}} l^r ( {\bf D}, {\bf c}|{\bf x}_t) + \alpha l^p ({\bf W}, {\bf c}|{\bf y}_t) +  
 \lambda_{c}||\boldsymbol{c}||_1,
 \end{eqnarray}
with $l^r$ being usually a sum-squared loss as in eq. \ref{eq. Lasso} and $l^p$ is the multinomial regression (cross-entropy) loss.

% The algorithm for online supervised dictionary learning works as follows:
% \begin{itemize}
% \item  initialize W and D
% \item  get new mini-batch of data sample (X,Y)
% \item for every new sample $\bs x_t$, compute code (hidden layer activation) for each (x,y) sample  \\ $c(x)  = \arg\ min Lp(W,c,y)  + \alpha Lr(D,c,x) + \lambda ||c_i||_1$, \\
% 	where Lp(W,c,y)  is the predictive loss (multinomial regression from c to y with parameters W). Solved by proximal method.
% \item update dictionary weights D as before in Alg 1 - block coordinate descent till convergence,
% using the objective in eq. 21
%                (note that the objective includes old data samples and  codes implicitly through memory matrices A and B
% \item update W - again, fitting multinomial regression from c to y, i.e. until convergence using multiple steps of
%               (stochastic) gradient  descent on W (well, it's essentially just gradient descent on current mini-batch as it is ran until convergence)
% end         
% \end{itemize}

\section{ Our Model: Online Supervised Deep Dictionary Learning}

We assuming the   loss functions $l^p$ and $l^r$ which correspond to the type of variables being reconstructed or predicted (i.e., real-valued variables are assumed to be Gaussian and associated with the sum-squared loss as in classical sparse coding, and the class label is typically a categoric variable associated with multinomial, or cross-entropy,  loss), e.g. 
    $ l^r ( {\bf D^{ij}},{\bf c^i}|{\bf c^j}) = ||{\bf c^j} -  D^{ij}{\bf c^i}||^2_2,$ and 
 $l^p ({\bf W^{i k+1}}, {\bf y}|{\bf c^i})    = multinomial ~ loss$.
 
  The algorithm for {\em online supervised deep dictionary learning} is shown in \algoref{alg:ODSDL}, assuming the architecture in Figure 1 (to be included: a multilayer model combining k levels of deep dictionary with the top supervised layer).
  
%\input{sec_alg_bullet_points.tex}
\input{sec_ODSDL_2pass_algorithm.tex}
  
At each iteration $t$, the next input sample $\bs{x}_t$  (or a batch of samples) is obtained. For each layer of hidden variables, $i$, from 1 to k,  we first obtain a sparse code ${\bf c}^i_t$  
 by solving via proximal method the objective in step \ref{as:sparse_coding}, assuming fixed dictionaries $\bs D^{i,0}$ and  $\bs D^{i,i-1}$ and fixed predictive weights $\bs W^{i,k+1}$.
Next,   both dictionaries are updated.

\noindent{\bf Dictionary update.} Let $\bs D$ denote $\bs D^{i,0}$ and  $\bs D^{i,i-1}$ at their update steps, respectively.  Note that, in order to prevent the dictionary entries from growing arbitrarily large, we follow \cite{mairal2009online} and impose the norm constraint, i.e. keep
  the columns of $\bs{D}$ within the convex set  $\mathcal{C}= \{\boldsymbol{D} \in \mathbb{R}^{m \times k} $ $~~s.t.~~ \forall j~ \boldsymbol{d}^T_j \boldsymbol{u}_j \leq 1 \}$. To update each dictionary, we optimize  the following {\em surrogate} objective function $\hat{f}_t({\bf D})$\footnote{this function is called surrogate since  each of the codes obtained on previous iterations $j < t$ are obtained using the corresponding earlier versions of the dictionary, rather than being computed with respect to the most recent dictionary, as in offline setting, and thus the surrogate function in online setting approximates the corresponding version in offline setting.}: 
%\vspace{-0.01in}
\begin{small}
\begin{equation}
\label{eqn:optimize_dict_obj_group_sparse}
\min_{\boldsymbol{D} \in \mathcal{C}}
\frac{1}{t} \sum_{j=1}^t \frac{1}{2}
||
\bs{c}^{i-1}_j - \boldsymbol{D} {\bs c}^i_j
||_2^2
+
\lambda_g \sum_j ||\boldsymbol{d}_j||_2
+
\sum_j\lambda_j||\boldsymbol{d}_j||_1.
%\vspace{-0.01in}
\end{equation}
\end{small}
Again, following \cite{mairal2009online}, we rewrite the above objective using the fact that $\min_{\boldsymbol{D} \in \mathcal{C}} \frac{1}{t}
\sum_{i=1}^t \frac{1}{2} ||
\boldsymbol{x}_i - \boldsymbol{D} \boldsymbol{\alpha}_i
||_2^2  $ is equivalent to   
\vspace{-0.05in}
\begin{eqnarray}
\label{eqn:optimize_dict_obj}
  \min_{\boldsymbol{D} \in \mathcal{C}}
\frac{1}{t} \big ( \frac{1}{2}
Tr(\boldsymbol{D}^T\boldsymbol{D}\boldsymbol{A}) - Tr(\boldsymbol{D}^T\boldsymbol{B}) \big ),
%\vspace{-0.02in}
\vspace{-0.05in}
\end{eqnarray}
  where $\bs{A} = \sum_{i=1}^t \boldsymbol{\alpha}_i \boldsymbol{\alpha}_i^T$ and $\bs{B} = \sum_{i=1}^t \boldsymbol{x}_i \boldsymbol{\alpha}_i^T$ are the ``bookkeeping''
  matrices (we also call them ``memories'' of the model), compactly representing the input samples and encoding history.
   At each iteration, once the new input sample $\boldsymbol{x}_i $ is encoded,
    the matrices are updated as $\boldsymbol{A} \gets \boldsymbol{A} + \boldsymbol{\alpha}_t \boldsymbol{\alpha}_t^T$ and $\boldsymbol{B}
\gets
\boldsymbol{B} + \boldsymbol{x}_t \boldsymbol{\alpha}_t^T$ (see the step \ref{as:memory_update}  of \algoref{alg:ODSDL}).
We follow \cite{mairal2009online} and use a \emph{block coordinate descent}   to optimize
 the convex objective
 in eq. \ref{eqn:optimize_dict_obj}; it iterates over the dictionary elements in a fixed sequence, until convergence, optimizing each while
 keeping the others fixed as shown in eq. \eqnref{eqn:dict_update}  and \ref{as:dict_element_normalize}  in \algoref{alg:ODSDL},
 except that, in our approach,
$\boldsymbol{u}_j$ is transformed into $\boldsymbol{w}_j$   to impose an additional regularizer before computing step \ref{as:dict_element_normalize}).
 
\begin{align}
\label{eqn:dict_update}
&
%\underbrace{
\boldsymbol{u}_j
\gets
\frac{
	\boldsymbol{b}_j
	-
	 \sum_{k \not = j} \boldsymbol{d}_k  a_{jk}
}
{
	a_{jj}
}
%}_{\text{minimize the least square error}}
;\ \ \
%\underbrace{
\boldsymbol{d}_j
\gets
\frac{
	\boldsymbol{u}_j
}
{
	\max(1, ||\boldsymbol{u}_j||_2)
}
\end{align}
 
\noindent{\bf Updating predictive weights $W^{i,k+1}$.} Finally,  step \ref{as:updateW}  in \algoref{alg:ODSDL} updates predictive (forward) weights ${\bf W}^{i,k+1}$ by fitting multinomial regression from code ${\bf c}^i_t$ to ${\bf y}_t$. Note that we have no obvious way to express the multinomial loss in terms of memory matrices as it was done for the sum-squared loss in eq. \ref{eqn:optimize_dict_obj}, and thus we will be using SGD instead of block-coordinate descent for this part of the loss function.



==> sec_introduction_old.tex <==
%\vspace{-0.1in}
\section{Introduction}
%\vspace{-0.1in}
\label{sec:intro}
 %%%
%  Our motivation - better training algorithms for deep networks, in both offline and online/continual/multi-task learning.

% 1. Why look beyond backprop?
The backpropagation algorithm has been the workhorse of neural net learning for several decades, since its  introduction in 1970s, and its practical effectiveness is demonstrated by recent   successes of deep learning in a wide range of applications. However, it has several drawbacks which continue to motivate research on alternative methods for neural net training.

One well-known problem with backpropagation (chain-rule differentiation)  is {\em vanishing gradients} \cite{hochreiter2001gradient}: recursive application of the chain rule through multiple layers of %compressing
nonlinearities causes the magnitudes of gradients to become very small in shallow layers, generating a weak error signal that slows convergence and  hampers learning, especially in very deep and/or recurrent networks \cite{bengio1994learning,riedmiller1993direct,hochreiter1997long, glorot2010understanding}.  Although various techniques were proposed to address this issue, including Long Short-Term Memory \cite{hochreiter1997long}, RPROP \cite{riedmiller1993direct}, rectified linear units (ReLU) \cite{nair2010rectified},  network architectures with
shorter input-to-output paths such as ResNet \citep{he2016deep},
the fundamental problem with computing gradients of a deeply nested objective function remains. 
Furthermore, {\em backpropagation can only handle differentiable nonlinearities} and it {\em does not parallelize over the network layers}. Finally, another commonly expressed  concern  about backpropagation is its  {\em biological implausibility}, including, among other issues,  deterministic (rather than stochastic) neurons, precise alternation between the feedforward and backpropagation phases, the requirement that the feedback path have exactly the same connectivity and symmetric weights (transposed) as the corresponding feedforward path, and the fact that the error propagation mechanism does not influence neural activity, unlike known biological feedback mechanisms \cite{lee2015difference,bartunov2018assessing}.
 
 %%%%%%%%%%%%%%%%%%

 % 2. New emergent research direction based on aux variables/variable splitting/ lifted approaches: alternative approaches involving auxiliary variables and breaking nested function optimization into a bunch of local optimization problems: BCD,MAC,target prop, etc
%State-of-art:

In order to overcome the vanishing gradient issue and others mentioned above, several approaches were proposed recently, based on the  idea of using auxiliary variables associated with hidden unit activations in order to decompose the  highly coupled problem of optimizing a  nested loss function  into  multiple, loosely coupled, simpler subproblems. Namely, given a network with $L$ hidden layers, and the output $y$, the standard formulation involves optimizing  the  loss function ${\cal{L}}(y,f({\bs W},\bs{x}_L))$ with respect to the network weights ${\bs W}$, where  $f({\bs W},\bs{x}_L)=f_{L+1}(\bs{W}_{L+1},f_L(\bs{W}_L,f_{L-1}(\bs{W}_{L-1},...f_1(\bs{W}_1,\bs{x})...)$
is a nested function associated with multilayer transformations in a  deep network. However, instead of solving the above problem, one can introduce auxiliary variables $\bs{x}_i, i=1,...,L$, and relax constraints ensuring that those variables   match the network transformations at each layer. Then the problem of  optimizing the loss with respect to both  the weights and auxiliary variables  decomposes   into multiple local subproblems, each involving only activations and weights within the two adjacent layers. Several methods based on auxiliary variables were proposed recently,  including   the alternating direction method of multipliers (ADMM) \cite{taylor2016training,zhang2016efficient} and block coordinate descent (BCD) methods \cite{zeng2018block,zhang2017convergent,Zhang2017,Askari2018,carreira2014distributed}. Empirical evaluation of these demonstrated  faster growth of their test accuracy as compared to SGD, due to parallel implementation;  moreover, these approaches avoid the vanishing gradient issue and can deal with non-differentiable functions, e.g.,  binarized neural networks \cite{courbariaux2015binaryconnect,hubara2016binarized}. Note that a similar formulation, using Lagrange multipliers,   was proposed  earlier in \cite{le1986learning,yann1987modeles,lecun1988theoretical}, where a constrained formulation involving activations required the output of the previous layer to be equal to the input of the next layer. This gave rise to the approach known as  target propagation and its recent extensions \cite{lee2015difference,bartunov2018assessing}; however, target propagation uses a different approach than iterative BCD and ADMM methods,  training instead layer-wise inverses of the forward mappings.

%3.  What's wrong with current AltMin methods?

While the BCD and ADMM methods discussed above assume an offline (batch) setting, i.e. the full training dataset being available at each iteration of the training phase, we will focus instead on the {\em online}, incremental learning approach, performing {\em alternating minimization (AM)} over the network weights and auxiliary activation variables, which we refer to as {\em online AM}. One advantage of the online approach is its natural ability to handle very large, practically unlimited, amounts of samples. Furthermore, unlike its offline counterparts, our approach  can  be applied to multi-task, {\em continual (lifelong) learning} problems, i.e.  online learning in nonstationary environments (though this is not the focus of current paper). 


 


Herein, we introduce two versions of online AM, one using SGD locally for weight updates in each layer (but without the need for chain computation of gradients due to separation into subproblems discussed above), and the second one, based on the   online learning approach similar to the online dictionary learning of \cite{mairal2009online}, that  relies on  accumulation of second-order information  which can be viewed as a ''memory'' of co-activations.

%among the units in the same layer, and across the adjacent layers (i.e., activation covariance and cross covariance matrices). Both proposed versions, called {\em online-AM-SGD} and {\em online-AM-BCD} (since the memory-based approach employed BCD within each layer optimization), demonstrate promising empirical results, clearly ouperforming    the corresponding  off-line alternating minimization, as well as closely related approach of \cite{taylor2016training}; furthermore, in some regimes/datasets, online AltMin outperforms backpropagation-SGD, while  being  comparable to the latter in other regimes and datasets.   Finally,  we provide novel theoretical convergence guarantees for general   alternating minimization schemes in online, stochastic settings.

Our contributions:
\begin{itemize}
    \item  online/mini-batch vs batch 
    \item for binary nets, no need for straight through estimator, since we can solve easier local subpropblems (similar to reLu)
    \item convex subproblems for weights
    \item less aux variables than ADMM
\end{itemize}

In summary, our contribution is a novel online  alternating minimization algorithm for neural net training,  utilizing auxiliary activation variables which break the gradient chain rule (unlike classical backpropagation) into independent local optimization subproblems, which is also equipped with a  theoretical convergence analysis, often performs similarly  or better  than its competitors, and possesses additional useful properties  lacking in  backpropagation, namely: (1)  {\em no vanishing  gradients}; (2) handling  {\em non-differentiable nonlinearities} more easily within layer-wise local subproblems;
(3)   possibility for {\em parallelization across  layers} for weight updates (similar to \cite{carreira2014distributed});  
(4) a {\em  more biologically plausible} credit assignment algorithm (local, parallel/distributed, stochastic, activation-based) as compared to  backpropagation;  (5) {\em co-activation memory mechanism} -- a novel feature arising from our online optimization approach; exploring  co-activation memory effects in  life-long learning is the direction of our ongoing work, although not the focus of this paper.
 

This paper is structured as follows. Section 2 introduces the optimization problem for online learning of a deep network with explicit activation  variables, and describes the proposed alternating minimization algorithm. Section 3 introduces theoretical results, while Section 4 presents empirical evaluation.  Section 5 concludes the paper with a summary and discussion of future work.



==> sec_our_algo_pseudo_code.tex <==
%\vspace{-0.05in}
\begin{small}
\begin{algorithm}[th]
\caption{
\fontsize{9}{9}\selectfont
 Neurogenetic Online Dictionary Learning (NODL)
}
\csize
\begin{algorithmic}[1]
\REQUIRE Data stream $\boldsymbol{x}_1, \bs{x}_2, \cdots, \bs{x}_n \in \mathbb{R}^m$; initial dictionary $\boldsymbol{D} \in \mathbb{R}^{m \times k}$; conditional neurogenesis threshold, $\gamma$; max number of new elements added per data batch,  $c_k$; group sparsity regularization parameter, $\lambda_g$; number of non-zeros in a dictionary element, $\beta_d$; number of non-zeros in a code, $\beta_c$.
%\newline
\STATE
Initialize: $\boldsymbol{A} \gets 0$, $\boldsymbol{B} \gets 0$~   \COMMENT{ reset the ``memory''}\\
\COMMENT{single data in a batch, for simpler exposition}
%\WHILE{there is a batch of data to process}
\FOR{$t = 1$ to $n$}
%\STATE
%{\bf Input} next batch  of data $\{ \boldsymbol{x}_1, \cdots,  \boldsymbol{x}_t, \cdots, \boldsymbol{x}_b \}$  \\
\STATE
Input $\boldsymbol{x}_t$\COMMENT{representing the $t_{th}$ batch of data}
\label{as:input_data}
\\
\COMMENT{Sparse coding of data:}
%\FOR{$t = 1$ to $b$}
\STATE
$
\boldsymbol{\alpha}_t
=
\arg_{\boldsymbol{\alpha} \in \mathbb{R}^k} \min
\frac{1}{2}
||
	\boldsymbol{x}_t - \boldsymbol{D} \boldsymbol{\alpha}
||^2_2
+
\lambda_c
||
\boldsymbol{\alpha}
||_1
$
\label{as:sparse_coding}
%\ENDFOR
\COMMENT{$\lambda_c$ tuned to have $\beta_c$ non-zeros in $\alpha_t$}
\\
\algshade{
\COMMENT{Conditional neurogenesis: if accuracy below threshold, add more elements
%~(should not be more than the number of data in a batch)
}
%\IF{$p_c(\boldsymbol{x}_1, \cdots, \boldsymbol{x}_b, \boldsymbol{D}, \boldsymbol{\alpha}_1,  \cdots, \boldsymbol{\alpha}_b) \leq \gamma$}
\IF{$p_c(\boldsymbol{x}_t, \boldsymbol{D}, \boldsymbol{\alpha}_t) \leq \gamma$}
\label{as:condition_neurogenesis}
\STATE $k_{n} = (1-p_c(\boldsymbol{x}_t, \boldsymbol{D}, \boldsymbol{\alpha}_t)) c_{k}$\COMMENT{
the count of the births
% of neurons
}
\label{as:num_new_neurons}
\STATE $\boldsymbol{D}_{n} \gets initializeRand(k_{n})$,
$
\\
\boldsymbol{D}
\gets
\left[
\begin{matrix}
\boldsymbol{D} & \boldsymbol{D}_{n}\\
\end{matrix}
\right]
$
\label{as:init_new_elements}
\STATE
$
\boldsymbol{A} \gets
\left[
\begin{matrix}
\boldsymbol{A} & \boldsymbol{0}\\
\boldsymbol{0} & \boldsymbol{0}\\
\end{matrix}
\right]
$,
 \
 $
 \boldsymbol{B}
 \gets
\left[
\begin{matrix}
\boldsymbol{B} & \boldsymbol{0}\\
\end{matrix}
\right]
 $,\ $k \gets k + k_{n}$
 \label{as:memory_increase}
 \\
\COMMENT{
Repeat sparse coding,
with the new elements
%now including the new dictionary elements
}
%\FOR{$t = 1 \to b$}
 \STATE
$
\boldsymbol{\alpha}_t
=
\arg_{\boldsymbol{\alpha} \in \mathbb{R}^k} \min
\frac{1}{2}
||
	\boldsymbol{x}_t - \boldsymbol{D} \boldsymbol{\alpha}
||^2_2
+
\lambda_c
||
\boldsymbol{\alpha}
||_1
$
\label{as:recompute_sparse_code}
%\ENDFOR
\ENDIF \COMMENT{End of neurogenesis}
%\\
} %end of algshade
\COMMENT{  ``Memory'' update:}
%\FOR{$t = 1 \to b$}
\STATE
$
\boldsymbol{A} \gets \boldsymbol{A} + \boldsymbol{\alpha}_t \boldsymbol{\alpha}_t^T
$,\ \
$
\boldsymbol{B} \gets \boldsymbol{B} + \boldsymbol{x}_t \boldsymbol{\alpha}_t^T
$
%\ENDFOR
\label{as:memory_update}
\\
\COMMENT{Dictionary update by block-coordinate descent
%with $l_1/l_2$ group sparsity
}
\REPEAT
\label{as:dict_update_repeat}
%\COMMENT{Update each dictionary element:}
\FOR{$j = 1$ to $k$}
\STATE
%\begin{align*}
%\vspace{-0.4in}
%&
$
\boldsymbol{u}_j
\gets
\frac{
	\boldsymbol{b}_j
	-
	 \sum_{k \not = j} \boldsymbol{d}_k  a_{jk}
}
{
	a_{jj}
}
$
\label{as:dict_element_compute}
%\\
%&
%\algshade{
\\
\algshade{
\COMMENT{Sparsifying elements~(optional):}
\STATE
%\begin{align*}
%\begin{align*}
$
\boldsymbol{v}_j
\gets
Prox_{\lambda_j ||.||_1}(\boldsymbol{u}_j)
=
sgn(\boldsymbol{u}_j) (|\boldsymbol{u}_j| - \lambda_j)_{+},
$\COMMENT{$\lambda_j$ tuned to get $\beta_d$ non-zeros in $\boldsymbol{v}_j$}
\label{as:sparse_elements}
%}
%\\
%&
\\
%\algshade{
\COMMENT{Killing useless elements with $l_1/l_2$ group sparsity}
\STATE
$
\boldsymbol{w}_j
\gets
\boldsymbol{v}_j
\left(
	1
	-
	\frac{\lambda_g}{||\boldsymbol{v}_j||_2}
\right)_{+}
$
}
\label{as:kill_elements}
\\
%\end{align*}
%}
%\STATE
%\begin{align*}
%&
\STATE
$
\boldsymbol{d}_j
\gets
\frac{
	\boldsymbol{w}_j
}
{
	\max(1, ||\boldsymbol{w}_j||_2)
}	
$
\label{as:dict_element_normalize}
%\end{align*}
%\vspace{-0.1in}
\ENDFOR
\UNTIL{\textbf{convergence}}
\label{as:dict_update_until_converge}
\ENDFOR
%\ENDWHILE
\RETURN $\boldsymbol{D}$
\end{algorithmic}
\label{alg:neurogen_mairal}
\end{algorithm}
\end{small}
%\vspace{-0.05in}


==> sec_related.tex <==
\section{Related Work}
\noindent{\bf From Fenchel Lifted Networks}

Lifted methods Related works that lift the dimension of the training problem are primarily optimized using BCD or ADMM. These methods have experienced recent success due to their ability to exploit the structure of the problem by first converting the constrained optimization problem into an unconstrained one and then solving the resulting sub-problems in parallel. They do this by relaxing the network constraints and introducing penalties into the objective function. The two main ways of introducing penalties into the objective function are either using quadratic penalties (Sutskever et al., 2013; Taylor et al., 2016; Lau et al.,
2018) or using equivalent representations of the activation functions (Askari et al., 2018; Zhang and Brand, 2017). As a result, these formulations have many advantages over the traditional training problem, giving superior performance in some specific network structures (Carreira-Perpinan and Wang, 2014; Zhang and
Brand, 2017). These methods also enjoy great potential to parallelize as shown by Taylor et al. (2016). However, there has been little evidence showing that these methods can compete with traditional DNNs which shadows the nice structure these formulations bring about. An early example of auxiliary variables being introduced into the training problem is the method of auxiliary coordinates (MAC) by Carreira-Perpinan and Wang (2014) which uses quadratic penalties to enforce network constraints. They test their method on auto encoders and show that their method is able to outperform SGD. Taylor et al. (2016) further extend this work by demonstrating the huge potential to parallelize these methods. Lau et al. (2018) gives some convergence guarantee on a modified problem.

Another class of models that lift the dimension of the problem do so by representing activation functions in equivalent formulations. Negiar et al. (2017); Askari et al. (2018); Zhang and Brand (2017) explore the structure of activation functions and use arg min maps to represent activation functions. In particular, Askari et al. (2018) show how a strictly monotone activation function can be seen as the arg min of a specific optimization problem. Just as with quadratic penalties, this formulation of the problem still performs poorly compared to traditional neural networks.

 

\noindent{\bf From LPOM paper}

Recently, many variants of SGD have been proposed, which use adaptive learning rates and momentum terms, e.g., Nesterov momentum (Sutskever et al., 2013), AdaGrad (Duchi, Hazan, and Singer, 2011), RMSProp (Dauphin, de Vries, and Bengio, 2015), and Adam (Kingma and Ba, 2014). SGD and its variants use a few training samples to estimate the full gradient, making the computational complexity of each iteration small. Moreover, the estimated gradients have noise, which is helpful for escaping saddle points (Ge et al., 2015).   However, they have some drawbacks as well. One major problem is the vanishing or blow-up gradient issue, where the magnitudes of gradients decrease or increase exponentially with the number of layers. This causes slow or unstable convergence, especially in very deep networks. This flaw can be remitted by using non-saturating activation functions, such as rectified linear unit (ReLU), and modified network architectures, such as ResNet (He et al., 2016). However, the fundamental problem remains. Also, their parameters are difficult to tune (e.g., learning rates and convergence criteria) (Le et al., 2011). Furthermore, they cannot deal with non-differentiable activation functions directly (e.g., binarized neural networks (Hubara et al., 2016)) and do not allow parallel weight updates across the layers (Le et al., 2011). For more on the limitations of SGD, please refer to (Taylor et al., 2016) and (Le et al., 2011). 


The drawbacks of SGD motivate research on alternative training methods for DNNs. Recently, training a feed-forward neural network is formulated as a constrained optimization problem, where the network activations are introduced as auxiliary variables and the network configuration is guaranteed by layer-wise constraints (Carreira-Perpinan and Wang, 2014). It breaks the dependency among the nested functions into equality constraints, so many standard optimization methods can be utilized. Some methods of this type of approach were studied and they differed in how to handle the equality constraints. Carreira-Perpinan and Wang (2014) approximated the equality constraints via quadratic penalties and alternately optimized network weights and activations. Zeng et al. (2018) introduced one more block of auxiliary variables per layer and also approximated the equality constraints via quadratic penalties. Inspired by alternating direction method of multiplier (ADMM) (Lin, Liu, and Su,
2011), Taylor et al. (2016) and Zhang, Chen, and Saligrama (2016) used the augmented Lagrangian approach to obtain exact enforcement of the equality constraints. However, the two methods involved the Lagrange multipliers and nonlinear constraints, thus were more memory demanding and more difficult in optimization. Motivated by the fact that the ReLU activation function is equivalent to a simple constrained convex minimization problem, Zhang and Brand (2017) relaxed the nonlinear constraints as penalties, which encode the network architecture and the ReLU activation function. Thus, the nonlinear constraints no longer exist. However, their approach is limited to the ReLU function and does not apply to other activation functions. Askari et al. (2018) followed this idea by considering more complex convex optimization problems and discussed several types of non-decreasing
activation functions. However, their methods to update the weights and activations are still limited to the ReLU function. Their approach cannot outperform SGD and can only serve for initializing SGD.

\noindent{\bf Details on AM-like methods}

By introducing the layer-wise activations as a block of auxiliary variables, the training of a neural network can be equivalently formulated as an equality constrained optimization problem (Carreira-Perpinan and Wang, 2014). The constraints ensure that the auxiliary variables  exactly match the forward pass of the network. Compared with problem (1), problem (2)
is constrained. But since the objective function is not nested, hence much simpler, such an equivalent reformulation may lead to more flexible optimization methods. Note that
when using SGD to solve problem (1), it actually works on problem (2) implicitly as the activations  need be recorded in order to compute the gradient.

 Zeng et al. (2018) decoupled the nonlinear activations in (2) with new auxiliary variables:
 
This is called as the 3-splitting formulation. Accordingly, problem (2) is the 2-splitting formulation.

They adapted a BCD method to solve the above problem. Taylor et al. (2016) also considered solving problem (4). Inspired by ADMM (Lin, Liu, and Su, 2011), they added a Lagrange multiplier to the output layer. Note that the activation function on the output layer is absent. So (6) is only a heuristic adaptation of
ADMM. 

Zhang, Chen, and Saligrama (2016) adopted a similar technique but used a different variable splitting scheme. Despite the nonlinear equality constraints, which ADMM is not designed to handle, they added a Lagrange multiplier
for each constraint. Their method is designed tpo learn hash functions.

Different from naively applying the penalty method and ADMM, Zhang and Brand (2017) interpreted the ReLU activation function as a simple smooth convex optimization
problem. Their penalty terms encode both the network structure and activation function. Unlike MAC and ADMM based methods, it does not include nonlinear activations. Moreover, the major advantage is that problem (10) is block multiconvex, i.e., the problem is convex w.r.t. each block of variables when the remaining blocks are fixed. They developed a new BCD method to solve it. They also empirically demonstrated the superiority of the proposed approach over SGD
based solvers in Caffe (Jia et al., 2014) and the ADMM based method (Zhang, Chen, and Saligrama, 2016). However, their approach is limited to ReLUs only, and empirical evaluation is limited to special skip-connection 3-layer net and MNIST. 

Askari et al.
(2018) inherited the same idea. By introducing a more complex convex minimization problem, they could handle more general activation functions.

LPOM (AAAI 2019)  is implemented in MATLAB and is not scalable to datasets like HIGGS. Their comparison is with plain SGD. 


 

 
\noindent{\bf Relation to equilibrium prop}

There is also a notable similarity between Initialized Equilibrium Propagation and Method of Auxiliary Coordinates (Carreira-Perpinan & Wang, 2014). In that paper, the authors propose a scheme for optimizing a layered feedforward network which consists of alternating optimization of the neural
activations (which can be parallelized across samples) and parameters (which can be parallelized across layers). In order to ensure that the layer activations zk remain close to what a feedforward network can compute, the objective includes a layerwise cost. However, they differ from our method in that their layer-activations  are calculated using backpropagation-based optimization. Taylor et al. (2016) do something similar with using
the Alternating Direction Method of Multipliers (ADMM), where Lagrange multipliers enforce the “layer matching” constraints exactly. 

Both methods, unlike Equilibrium Prop, are full-batch methods.


\noindent{\bf LPOM method.}  We propose a new optimization method for training feed-forward neural networks. By rewriting the activation function as an equivalent proximal operator, we
approximate a feed-forward neural network by adding the proximal operators to the objective function as penalties, hence we call the lifted proximal operator machine (LPOM). LPOM is block multi-convex in all layer-wise
weights and activations. This allows us to use block coordinate descent to update the layer-wise weights and activations. Most notably, we only use the mapping of the activation function itself, rather than its derivative,
thus avoiding the gradient vanishing or blow-up issues in gradient based training methods. So our method is applicable to various non-decreasing Lipschitz continuous activation functions, which can be saturating and
non-differentiable.  Our method does not require more auxiliary variables than the layer-wise activations, thus using roughly the same amount of memory as stochastic gradient descent (SGD) does.   We further prove the convergence of updating the layer-wise weights and activations and point out that the optimization could be made parallel by asynchronous update. Experiments on MNIST and CIFAR-10 datasets ...

--------

Our first method falls into the class of online algorithms based on stochastic approximations, processing one sample at a time, but exploits the specific structure of the problem to efficiently solve it. Contrary to classical first-order stochastic gradient descent, it does not require explicit learning rate tuning and minimizes a sequentially quadratic local approximations of the expected cost.

---------

Non-SGD methods for deep learning were also studied in the recent years.
Taylor et al. proposed the Alternating Direction Method of Multipliers (ADMM)
to transform a fully-connected neural network into an equality-constrained problem to solve [33]. Zhang et al. [43] handled deep supervised hashing (VDSH)
problem by an ADMM algorithm to overcome vanishing gradients. Carreira and
Wang proposed a method of auxiliary coordinates (MAC) to replace a nested
neural network with a constrained problem without nesting [8].

 


\noindent{\bf Relation to target prop}

More broadly, other approaches to backprop-free credit assignment have been tried. Difference Target propagation (Lee et al., 2015) proposes a mechanism to send back targets to each layer, such that locally optimizing targets also optimizes the true objective. Feedback-Alignment (Lillicrap et al., 2014) shows that, surprisingly, it is possible to train while using random weights for the backwards pass in backpropagation, because the forward pass parameters tends to “align” to the backwards-pass parameters so that the pseudogradients tend to be within 90◦ of the true gradients. A similar phenomenon was observed in Equilibrium Propagation by Scellier et al. (2018), who showed that when one removed the constraint of symmetric weight in Equilibrium propagation, the weights would evolve towards symmetry through training. Finally, Jaderberg et al. (2016) used a very different approach - rather than create local targets, each layer predicts its own “pseudogradient”. The gradient prediction parameters are then trained either by the true gradients (which no longer need to arrive before a parameter update takes place) or by backpropagated versions of pseudogradients
from higher layers.

==> sec_related_general.tex <==
Synthetic Gradients:  individual layers instead make a "best guess" for what they think the data will say, and then update their weights according to this guess. This "best guess" is called a Synthetic Gradient. The data is only used to help update each layer's "guesser" or Synthetic Gradient generator. This allows for (most of the time), individual layers to learn in isolation, which increases the speed of training.

https://arxiv.org/abs/1703.00522
@article{czarnecki2017understanding,
  title={Understanding synthetic gradients and decoupled neural interfaces},
  author={Czarnecki, Wojciech Marian and {\'S}wirszcz, Grzegorz and Jaderberg, Max and Osindero, Simon and Vinyals, Oriol and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1703.00522},
  year={2017}
}

@article{zeng2018block,
  title={Block Coordinate Descent for Deep Learning: Unified Convergence Guarantees},
  author={Zeng, Jinshan and Lau, Tim Tsz-Kit and Lin, Shaobo and Yao, Yuan},
  journal={arXiv preprint arXiv:1803.00225},
  year={2018}
}

@inproceedings{suzuki2013dual,
  title={Dual averaging and proximal gradient descent for online alternating direction multiplier method},
  author={Suzuki, Taiji},
  booktitle={International Conference on Machine Learning},
  pages={392--400},
  year={2013}
}
http://proceedings.mlr.press/v28/suzuki13.pdf


-----------------------------
Alternating minimization for dictionary learning with random initialization
http://papers.nips.cc/paper/6795-alternating-minimization-for-dictionary-learning-with-random-initialization

Deep Dictionary Learning paper:
http://ieeexplore.ieee.org/document/7779008/


Deep Dictionary Learning vs Deep Belief Network vs Stacked Autoencoder: An Empirical Analysis
https://link.springer.com/chapter/10.1007/978-3-319-46681-1_41

How to Train Your Deep Neural Network with Dictionary Learning
https://arxiv.org/abs/1612.07454

Greedy Deep Dictionary Learning
https://arxiv.org/abs/1602.00203
 -----------
How Auto-Encoders Could Provide Credit Assignment in Deep Networks via Target Propagation 
https://arxiv.org/pdf/1407.7906.pdf


Deconstructing the Ladder Network Architecture 
https://arxiv.org/pdf/1511.06430.pdf

Augmenting Supervised Neural Networks with Unsupervised Objectives for Large-scale Image Classification 
http://proceedings.mlr.press/v48/zhangc16.pdf

Supervised Deep Sparse Coding Networks 
https://arxiv.org/pdf/1701.08349.pdf


"We conduct extensive experiments on CIFAR-10, CIFAR-100, STL-10 and MNIST. We demonstrate that the proposed SCN exhibits competitive performance while using much smaller number of parameters and layers compared to numerous deep neural network approaches. Notably, a 14- layer SCN model exceeds the performance of a 164-layer and 1001-layer deep residual network, respectively " 


----------
 
AltMin-like (block-coordinate descent etc) algorithms:

 
https://arxiv.org/pdf/1706.04638.pdf

Proposition 1 in the paper is quite interesting: it shows that gradient descent on a standard neural network and gradient descent on a quadratically penalized loss (what Carreira-Perpiñán uses in the method of auxiliary coordinates) are equivalent.


1.  Convergent Block Coordinate Descent for Training Tikhonov Regularized Deep Neural Networks 
https://arxiv.org/pdf/1711.07354.pdf
 
2. Difference target propagation
@inproceedings{lee2015difference,
 title={Difference target propagation},
 author={Lee, Dong-Hyun and Zhang, Saizheng and Fischer, Asja and Bengio, Yoshua},
 booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
 pages={498--515},
 year={2015},
 organization={Springer}
}

3.  Method of Auxiliary Variables (MAC)
4. ADMM
 

--------
Papers involving  skip connections in  deep nets:

Another (very empirical) paper on skip-connections:  https://arxiv.org/abs/1712.09913

Densely connected convolutional networks
@article{huang2016densely,
 title={Densely connected convolutional networks},
 author={Huang, Gao and Liu, Zhuang and Weinberger, Kilian Q and van der Maaten, Laurens},
 journal={arXiv preprint arXiv:1608.06993},
 year={2016}
}

Semi-Supervised Learning with Ladder Networks
@inproceedings{rasmus2015semi,
 title={Semi-supervised learning with ladder networks},
 author={Rasmus, Antti and Berglund, Mathias and Honkala, Mikko and Valpola, Harri and Raiko, Tapani},
 booktitle={Advances in Neural Information Processing Systems},
 pages={3546--3554},
 year={2015}
} 
Training Very Deep Networks ("Highway networks")
@inproceedings{srivastava2015training,
 title={Training very deep networks},
 author={Srivastava, Rupesh K and Greff, Klaus and Schmidhuber, J{\"u}rgen},
 booktitle={Advances in neural information processing systems},
 pages={2377--2385},
 year={2015}
}

Deep Residual Learning for Image Recognition
@inproceedings{he2016deep,
 title={Deep residual learning for image recognition},
 author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
 booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
 pages={770--778},
 year={2016}
}

3. Deep dictionary learning
Unsupervised Feature Learning by Deep Sparse Coding
Nonlinear dictionary learning based deep neural networks
How to Train Your Deep Neural Network with Dictionary Learning
Deep dictionary learning

4. supervised dict learning

J. Mairal, F. Bach, J. Ponce, G. Sapiro and A. Zisserman. Supervised Dictionary Learning. Advances in Neural Information Processing Systems (NIPS), 2008. [pdf]
I. Rish, G. Grabarnik, G. Cecchi, F. Pereira, G. Gordon Closed-form supervised dimensionality reduction with generalized linear models ICML 2008 

J. Mairal, F. Bach, J. Ponce. Task-DrivenDictionary Learning. Technical report, HAL : inria-00521534, 2010. [pdf]

Gangeh, M. J., Ghodsi, A., & Kamel, M. S. (2013). Kernelized supervised dictionary learning. IEEE Transactions on Signal Processing, 61(19), 4753-4767.


S. Kong and D. Wang. Online Discriminative Dictionary Learning for Image Classification Based on Block-Coordinate Descent Method. arXiv 2012

G Zhang, Z Jiang, LS Davis. Online semi-supervised discriminative dictionary learning for sparse representation, Asian Conference on Computer Vision, 2012

Yuxin Zhang and Bo Yuan. Supervised Online Dictionary Learning for Image Separation Using OMP, ICIC-2016 


